The cycle double cover conjecture from the perspective of percolation theory on iterated line graphs

The cycle double cover conjecture is a long standing problem in graph theory, which links local properties, the valency of a vertex and no bridges, and a global property of the graph, being covered by a particular set of cycles. We prove the conjecture using a lift of walks and cycles in $G$ to sets of open and closed edges on $\mathcal{L}(\mathcal{L}(G))$, the line graph of the line graph of $G$. We exploit that triangles are preserved by the line graph operator to obtain a one-to-one mapping from walks in the underlying graph $G$ to walks on $\mathcal{L}(\mathcal{L}(G))$. We prove that each set of "double walk covers" in $G$ induces a certain set of $\lbrace 0,1\rbrace$ labels on a subgraph covering of $\mathcal{L}(\mathcal{L}(G))$, minus a set of triangles, and conversely, that there is such a set of labels such that its projection back to $G$ implies a double cycle cover, if $G$ is an simple bridgeless triangle-free cubic graph. The techniques applied are inspired by percolation theory, flipping the $\lbrace 0,1\rbrace$ labels to obtain the desired structure.

==> chapters/SNMaEP_IAE.tex <==
In this section we are going to establish basic properties of $\mathfrak{S}_k$ independent of the graph structure as long as $L$ is a connected simple graph. 
\vspace{5pt}
\begin{tcolorbox}[boxsep=0pt,arc=0pt,colback=burgundy!15!white, frame empty]%%
	\begin{theorem}\label{thm:S_irred_aperiodic}
 		The Markov chain $\mathfrak{S}_k$ on $\mathfrak{L}_k$ is irreducible and aperiodic. 
 	\end{theorem}
 \end{tcolorbox}
 	\begin{proof}
 		Let $\mathfrak{v},\mathfrak{w}\in \mathfrak{V}_k$ such that $p_{k;\mathfrak{v},\mathfrak{w}}^{\triangle}>0$. Then also $p_{k;\mathfrak{w},\mathfrak{v}}^{\triangle}>0$ even though equality is not necessarily satisfied. Furthermore every $\langle \mathfrak{w},\mathfrak{v}\rangle\in \mathfrak{E}_k$ implies that $p_{k;\mathfrak{v},\mathfrak{w}}^{\triangle}>0$. Since $\mathfrak{L}_k$ is connected by Proposition \ref{prop:L_frak_k_connected} we obtain that the chain is irreducible.\\ 
 		The aperiodicity of $\mathfrak{S}_k$ follows directly from the fact that we can construct a state $\mathfrak{v}\in \mathfrak{V}_k$ such that $p_{k;\mathfrak{v},\mathfrak{v}}^{\triangle}>0$.
 	\end{proof}
By Theorem \ref{thm:convergence_to_stat_dist_irred_aperiod} on Markov chains on finite state spaces, we can conclude from Theorem \ref{thm:S_irred_aperiodic} that $\mathfrak{S}_k$ is ergodic, i.e., there is a stationary distribution and the chain converges independently of its initial distribution to said stationary distribution. 
\vspace{5pt}
\begin{tcolorbox}[boxsep=0pt,arc=0pt,colback=burgundy!15!white, frame empty]%%
	\begin{theorem}\label{thm:S_existence_stat_dist}
 		Let $L=(V,E)$ be a $\bar{d}$-regular graph, $\bar{n}:=|V|$ and $k\in\{1,\hdots,\bar{n}-1\}$. Let $\mathfrak{L}_k=(\mathfrak{V}_k, \mathfrak{E}_k)$ be defined as in Definition \ref{def:mathfrak_L_k}. Then there exists a distribution $\tilde{\pi}_k$ on $\mathfrak{V}_k$ such that the Markov chain $\mathfrak{S}_k$ converges in distribution to $\tilde{\pi}_k$ independently of its initial distribution $\nu_0$. 
 	\end{theorem}
\end{tcolorbox}
Having found an answer to this classical question we can wonder about the structure of $\tilde{\pi}_k$ as a function of $L$ and other properties of $\mathfrak{S}_k$ which govern the long-time behavior, like reversibility. While the classical exclusion process is always reversible, it turns out the choice exclusion process implies a structure on the transition matrix of $\mathfrak{S}_k$ which is only reversible in rare cases. The echo chamber model, therefore, gives rise to a qualitatively different kind of exclusion process as has been investigated before. 
\subsubsection{Lumpability and isomorph bipartite sub-graphs}\label{subsubsec:lumpability_isom}
In this subsection we are going to develop the idea of lumping the state space in detail, as defined in Definition \ref{def:lumpability_markov_chains} Due to the sensitivity of the Markov chain $\mathfrak{S}_k$ with respect to the number of particles as well as the geometry of the underlying graph, we have to apply sensitive tools based on as much information as possible from each sub-graph induced by a set of particles $\mathfrak{v}\in\mathfrak{V}_k$. It turns out that the bipartite sub-graphs $L_{\mathfrak{v},\mathfrak{v}^c}$ play an essential role. In fact, they provide a stronger form of lumpability for $\mathfrak{S}_k$ when lumping with respect to the degree of $\mathfrak{v}$ in $\mathfrak{L}_k$ is not possible, i.e., in almost all non-reversible cases.
\vspace{5pt}
\begin{tcolorbox}[boxsep=0pt,arc=0pt,colback=burntorange!25!white, frame empty]%%
	\begin{proposition}\label{prop:isom_of_bipartites_implies_same_transition_vect}
		Let $k\in\left\{1,\hdots,\bar{n}-1\right\}$ and let $\mathfrak{v}, \mathfrak{w} \in \mathfrak{V}_k$. Consider the by decreasing size ordered vectors $(p^{\triangle}_{k;\mathfrak{v},\mathfrak{u}})_{\mathfrak{u}\in\mathfrak{V}_k}$, $(p^{\triangle}_{k;\mathfrak{w},\mathfrak{u}})_{\mathfrak{u}\in\mathfrak{V}_k}$, $(p^{\triangle}_{k;\mathfrak{u},\mathfrak{v}})_{\mathfrak{u}\in\mathfrak{V}_k}$ and $(p^{\triangle}_{k;\mathfrak{u},\mathfrak{w}})_{\mathfrak{u}\in\mathfrak{V}_k}$. Then, $L_{\mathfrak{v},\mathfrak{v}^c}\stackrel{\sim}{=} L_{\mathfrak{w},\mathfrak{w}^c}$ if and only if these vectors satisfy the identities
		\begin{align*}
			(p^{\triangle}_{k;\mathfrak{v},\mathfrak{u}})_{\mathfrak{u}\in\mathfrak{V}_k}=(p^{\triangle}_{k;\mathfrak{w},\mathfrak{u}})_{\mathfrak{u}\in\mathfrak{V}_k}\\
			(p^{\triangle}_{k;\mathfrak{u},\mathfrak{v}})_{\mathfrak{u}\in\mathfrak{V}_k}=(p^{\triangle}_{k;\mathfrak{u},\mathfrak{w}})_{\mathfrak{u}\in\mathfrak{V}_k}.
		\end{align*}
	\end{proposition}
\end{tcolorbox}
\begin{proof}
	The claim follows since the bipartite graphs are isomorphic and, hence, any transition from or to $\mathfrak{v}$, defined by an edge from $\mathfrak{v}$ to $\mathfrak{v}^c$ can be translated to a transition from $\mathfrak{w}$ to $\mathfrak{w}^c$. In particular, assuming that $v\in\mathfrak{v}$ makes the transition, the number of neighbors is given by $\bar{d}-\mathrm{deg}^{L_{\mathfrak{v}}}(v)$ again using the isomorphism between $L_{\mathfrak{v},\mathfrak{v}^c}$ and $L_{\mathfrak{w},\mathfrak{w}^c}$ there is a unique $w\in\mathfrak{w}$ with $\bar{d}-\mathrm{deg}^{L_{\mathfrak{v}}}(v)$ neighbors. Consequently, for any transition probability $p^{\triangle}_{k;\mathfrak{v},\mathfrak{u}}$ we can construct a transition from $\mathfrak{w}$ to some neighbor such that $p^{\triangle}_{k;\mathfrak{v},\mathfrak{u}} = p^{\triangle}_{k;\mathfrak{v},\mathfrak{u}}$. Therefore, we obtain $(p^{\triangle}_{k;\mathfrak{v},\mathfrak{u}})_{\mathfrak{u}\in\mathfrak{V}_k}=(p^{\triangle}_{k;\mathfrak{w},\mathfrak{u}})_{\mathfrak{u}\in\mathfrak{V}_k}$.\par 
	Since $L_{\mathfrak{v},\mathfrak{v}^c}$ defines the whole neighborhood of $\mathfrak{v}$ in $\mathfrak{L}_k$ the converse for $(p^{\triangle}_{k;\mathfrak{u},\mathfrak{v}})_{\mathfrak{u}\in\mathfrak{V}_k}=(p^{\triangle}_{k;\mathfrak{u},\mathfrak{w}})_{\mathfrak{u}\in\mathfrak{V}_k}$ is also true.\par
	The inverse direction is true since the transition probabilities $p^{\triangle}_{k;\mathfrak{v},\mathfrak{u}}$ uniquely define the number of particles in the neighborhood of any particle $v\in\mathfrak{v}$ and the inverse direction $p^{\triangle}_{k;\mathfrak{u},\mathfrak{v}}$ defines all neighbors of $\mathfrak{v}$ which can be created by displacing a single particle $v$. Consequently, the whole vectors $(p^{\triangle}_{k;\mathfrak{v},\mathfrak{u}})_{\mathfrak{u}\in\mathfrak{V}_k}$ and $(p^{\triangle}_{k;\mathfrak{u},\mathfrak{v}})_{\mathfrak{u}\in\mathfrak{V}_k}$ define all possible transitions and, hence, the bipartite graph $L_{\mathfrak{v},\mathfrak{v}^c}$. Consequently, if the vectors coincide for $\mathfrak{v},\mathfrak{w}\in\mathfrak{V}_k$, then, we obtain $L_{\mathfrak{v},\mathfrak{v}^c}\stackrel{\sim}{=} L_{\mathfrak{w},\mathfrak{w}^c}$.
\end{proof}
Hence, two configurations $\mathfrak{v},\mathfrak{w}$ which satisfy  $L_{\mathfrak{v},\mathfrak{v}^c}\stackrel{\sim}{=} L_{\mathfrak{w},\mathfrak{w}^c}$ are seen as identical when it comes to transitions for the Markov chain $\mathfrak{S}_k$. Additionally, by defining the equivalence relation $\mathfrak{v}\sim \mathfrak{w}$ if and only if $L_{\mathfrak{v},\mathfrak{v}^c}\stackrel{\sim}{=} L_{\mathfrak{w},\mathfrak{w}^c}$ and using Lemma \ref{lem:isom_of_bipartites_implies_same_transition_proba} as well as Proposition \ref{prop:isom_of_bipartites_implies_same_transition_vect} we find that for a fixed $\mathfrak{v}\in\mathfrak{V}_k$ and $\mathfrak{w}\in\mathfrak{V}_k$ such that $L_{\mathfrak{v},\mathfrak{v}^c}\stackrel{\sim}{=} L_{\mathfrak{w},\mathfrak{w}^c}$ we have the identity $|\{\mathfrak{u}\in\mathfrak{V}_k|\mathfrak{u}\sim \mathfrak{v},\;\langle \mathfrak{u}, \mathfrak{v} \rangle\in\mathfrak{E}_k \}| = |\{\mathfrak{u}'\in\mathfrak{V}_k|\mathfrak{u}'\sim \mathfrak{w},\;\langle \mathfrak{u}', \mathfrak{w} \rangle\in\mathfrak{E}_k \}|$ and there is a bijection $\Phi:\{\mathfrak{u}\in\mathfrak{V}_k|\mathfrak{u}\sim \mathfrak{v},\;\langle \mathfrak{u}, \mathfrak{v} \rangle\in\mathfrak{E}_k \} \to \{\mathfrak{u}'\in\mathfrak{V}_k|\mathfrak{u}'\sim \mathfrak{w},\;\langle \mathfrak{u}', \mathfrak{w} \rangle\in\mathfrak{E}_k \}$ such that $ p^{\triangle}_{k;\mathfrak{v},\mathfrak{u}}=p^{\triangle}_{k;\mathfrak{w},\Phi(\mathfrak{u})}$. This leads us to the realization that $\sum_{\mathfrak{u}\sim \mathfrak{v}} p^{\triangle}_{k;\mathfrak{v},\mathfrak{u}} =\sum_{\mathfrak{u}'\sim \mathfrak{w}} p^{\triangle}_{k;\mathfrak{w},\mathfrak{u}'}$ which forms the basis for the following central result.
\vspace{5pt}
\begin{tcolorbox}[boxsep=0pt,arc=0pt,colback=burgundy!15!white, frame empty]%%
	\begin{theorem}\label{thm:natural_lumping_of_L_k_for_S_k}
		Let $L=(V,E)$ be a $\bar{d}$-regular graph with $\bar{n}=|V|$ and $k\in\left\{1,\hdots,\bar{n}-1\right\}$. Denote by $\mathfrak{L}_k=(\mathfrak{V}_k,\mathfrak{E}_k)$ the $k$-particle graph and define for $\mathfrak{v},\mathfrak{w}\in\mathfrak{V}_k$ the equivalence relation $\mathfrak{v}\sim\mathfrak{w}$ if and only if $L_{\mathfrak{v},\mathfrak{v}^c}\stackrel{\sim}{=} L_{\mathfrak{w},\mathfrak{w}^c}$. For fixed $\mathfrak{v}$ define $[\mathfrak{v}_i]:=\{\mathfrak{u}\in\mathfrak{V}_k|\mathfrak{u}\sim\mathfrak{v}_i\}$ the equivalence class of $\mathfrak{v}_i$ and denote by $l$ the number of distinct equivalence classes. Then, the Markov chain $\mathfrak{S}_k$ is strongly lumpable with respect to the partition $\{[\mathfrak{v}_1],\hdots,[\mathfrak{v}_l]\}$. 
	\end{theorem}
\end{tcolorbox}
\begin{proof}
	We have to show that for any $\mathfrak{w}_1,\mathfrak{w}_2 \in [\mathfrak{v}_i]$ 
	\begin{equation*}
		\sum_{\mathfrak{u}\in [\mathfrak{v}_j]} p^{\triangle}_{k;\mathfrak{w}_1,\mathfrak{u}} = 	\sum_{\mathfrak{u}\in \mathfrak{u}\in [\mathfrak{v}_j]} p^{\triangle}_{k;\mathfrak{w}_2,\mathfrak{u}}.
	\end{equation*}
	The equality follows directly by Proposition \ref{prop:isom_of_bipartites_implies_same_transition_vect} and the following observation. For $\mathfrak{w}_1,\mathfrak{w}_2\in [\mathfrak{v}_i]$ and $\mathfrak{u}_1\in [\mathfrak{v}_j]$ with $\langle \mathfrak{w}_1,\mathfrak{u}_1\rangle\in\mathfrak{E}_k$ we have $\mathfrak{w}_1\triangle\mathfrak{u}_1=\{w,u\}$. Let $\Phi$ be the isomorphism between $L_{\mathfrak{w}_1,\mathfrak{w}_1^c}$ and $L_{\mathfrak{w}_2,\mathfrak{w}_2^c}$. There is a unique edge in $L_{\mathfrak{w}_2,\mathfrak{w}_2^c}$, namely $\langle \Phi(w),\Phi(u) \rangle$, $\mathrm{deg}^{L_{\mathfrak{w}_1}}(w)=\mathrm{deg}^{L_{\mathfrak{w}_2}}(\Phi(w))$ and for $\mathfrak{u}_2:= (\{\Phi(w_1)|w_1\in\mathfrak{w}_1\}\backslash \Phi(w))\cup\{\Phi(u)\}$ we have $\mathfrak{u}_1\sim \mathfrak{u}_2$ by construction. Consequently, for any summand in the first sum, we find a corresponding summand in the second sum and vice versa such that they are equal.    
\end{proof}
Lumpability gives rise to the possibility to consider the Markov chain on a smaller state space and in an aggregated form. While, usually, this makes it impossible to make local statements for example on the specific value of $\tilde{\pi}_k(\mathfrak{v})$ for some $\mathfrak{v}\in\mathfrak{V}_k$ about $\mathfrak{S}_k$ based on the lumped chain, the stronger form of lumpability implied by Lemma \ref{prop:isom_of_bipartites_implies_same_transition_vect} allows to formulate further deductions. A central one is the structure of the stationary distribution $\tilde{\pi}_k$ of $\mathfrak{S}_k$. 
\vspace{5pt}
\begin{tcolorbox}[boxsep=0pt,arc=0pt,colback=burgundy!15!white, frame empty]%%
	\begin{theorem}\label{thm:stationary_dist_level_sets_pi_k}
		Let $L=(V,E)$ be a $\bar{d}$-regular graph with $\bar{n}=|V|$ and $k\in\left\{1,\hdots,\bar{n}-1\right\}$. Denote by $\tilde{\pi}_k$ the stationary distribution of $\mathfrak{S}_k$. Then, for all equivalence classes $[\mathfrak{v}]$ under the equivalence relation $\sim$ defined in Theorem \ref{thm:natural_lumping_of_L_k_for_S_k} all $\mathfrak{v},\mathfrak{w}\in[\mathfrak{v}]$ satisfy the identity $\tilde{\pi}_k(\mathfrak{v})=\tilde{\pi}_k(\mathfrak{w})$.
	\end{theorem}
\end{tcolorbox}
We are going to present, first, an intuitive approach, which is based on the idea that by Proposition \ref{prop:isom_of_bipartites_implies_same_transition_vect} two equivalent vertices $\mathfrak{v},\mathfrak{w}\in\mathfrak{V}_k$ are "identical" when it comes to their respective probability in- and out-"flow" and the approach that the equality of the average $|[\bar{\mathfrak{v}}]|^{-1}\tilde{\pi}_k([\bar{\mathfrak{v}}])$ and $\tilde{\pi}_k(\mathfrak{w})$ for an arbitrary $\mathfrak{w}\in[\bar{\mathfrak{v}}]$ gives the claim we are looking for. The following calculations are only correct under the assumption that for any $\mathfrak{v},\mathfrak{w}\in[\bar{\mathfrak{v}}]$ we have for any equivalence class $[\bar{\mathfrak{u}}]$ the identity 
\begin{equation}\label{eq:heuristic_statement_equality_v_to_w_change}
	\sum_{\mathfrak{u}\in[\bar{\mathfrak{u}}]}\tilde{\pi}_k(\mathfrak{u})p^{\triangle}_{k;\mathfrak{u},\mathfrak{v}} = \sum_{\mathfrak{u}\in[\bar{\mathfrak{u}}]}\tilde{\pi}_k(\mathfrak{u})p^{\triangle}_{k;\mathfrak{u},\mathfrak{w}}.
\end{equation}  
While there are $\mathfrak{u},\mathfrak{u}'\in[\bar{\mathfrak{u}}]$ such that the equality $p^{\triangle}_{k;\mathfrak{u},\mathfrak{v}}=p^{\triangle}_{k;\mathfrak{u}',\mathfrak{w}}$ is satisfied we cannot make a similar claim about $\tilde{\pi}_k(\mathfrak{u})p^{\triangle}_{k;\mathfrak{u},\mathfrak{v}}$ and $\tilde{\pi}_k(\mathfrak{u}')p^{\triangle}_{k;\mathfrak{u}',\mathfrak{w}}$. This leads to a recursive statement where the truth of the claim for one equivalence class $[\bar{\mathfrak{v}}]$ depends on the truth of the claim for all neighboring equivalence classes $[\bar{\mathfrak{u}}]$. Assuming, then, \ref{eq:heuristic_statement_equality_v_to_w_change} is satisfied we obtain for a fixed $\mathfrak{w}\in[\bar{\mathfrak{v}}]$
\begin{align*}
	\tilde{\pi}_k([\bar{\mathfrak{v}}]) &=\sum_{[\bar{\mathfrak{u}}]\in\faktor{\mathfrak{V}_k}{\sim}}\tilde{\pi}_k([\bar{\mathfrak{u}}])\hat{p}_{[\bar{\mathfrak{u}}],[\bar{\mathfrak{v}}]}=\sum_{[\bar{\mathfrak{u}}]\in\faktor{\mathfrak{V}_k}{\sim}}\sum_{\mathfrak{u}\in[\bar{\mathfrak{u}}]}\tilde{\pi}_k(\mathfrak{u})\sum_{\mathfrak{v}\in[\bar{\mathfrak{v}}]} p^{\triangle}_{k,\mathfrak{u},\mathfrak{v}}\\
	&=\sum_{[\bar{\mathfrak{u}}]\in\faktor{\mathfrak{V}_k}{\sim}}\sum_{\mathfrak{u}\in[\bar{\mathfrak{u}}]}\sum_{\mathfrak{v}\in[\bar{\mathfrak{v}}]} \tilde{\pi}_k(\mathfrak{u})p^{\triangle}_{k,\mathfrak{u},\mathfrak{v}}=\sum_{[\bar{\mathfrak{u}}]\in\faktor{\mathfrak{V}_k}{\sim}}\sum_{\mathfrak{v}\in[\bar{\mathfrak{v}}]}\sum_{\mathfrak{u}\in[\bar{\mathfrak{u}}]} \tilde{\pi}_k(\mathfrak{u})p^{\triangle}_{k,\mathfrak{u},\mathfrak{v}}\\
	&\stackrel{\ref{eq:heuristic_statement_equality_v_to_w_change}}{=}\sum_{[\bar{\mathfrak{u}}]\in\faktor{\mathfrak{V}_k}{\sim}}\sum_{\mathfrak{v}\in[\bar{\mathfrak{v}}]}\sum_{\mathfrak{u}\in[\bar{\mathfrak{u}}]} \tilde{\pi}_k(\mathfrak{u})p^{\triangle}_{k,\mathfrak{u},\mathfrak{w}}=|[\bar{\mathfrak{v}}]|\sum_{\mathfrak{u}\in\mathfrak{V}_k} \tilde{\pi}_k(\mathfrak{u})p^{\triangle}_{k,\mathfrak{u},\mathfrak{w}}=|[\bar{\mathfrak{v}}]|\tilde{\pi}_k(\mathfrak{w}).
\end{align*}
This would lead to the claim of Theorem \ref{thm:stationary_dist_level_sets_pi_k} but the problem now lies in proving \ref{eq:heuristic_statement_equality_v_to_w_change}. This poses, again, a recursive problem in terms of the neighborhoods of each $\mathfrak{v}\in[\bar{\mathfrak{v}}]$ which is due to the missing information on the local structure of $\mathfrak{L}_k$ inaccessible. Indeed, we need a global perspective on $\mathfrak{L}_k$, which is based on cycles and their identification for equivalent vertices $\mathfrak{v},\mathfrak{w}$, where we denote the equivalence relation by $\sim$.
\begin{lemma}\label{lem:cycle_identifiation_on_equi_class}
	Let $L=(V,E)$ be a $\bar{d}$-regular graph and $\mathfrak{v},\mathfrak{w}\in\mathfrak{V}_k$. Define for $\mathfrak{v},\mathfrak{w}\in\mathfrak{V}_k$ the equivalence relation $\mathfrak{v}\sim\mathfrak{w}$ if and only if $L_{\mathfrak{v},\mathfrak{v}^c}\stackrel{\sim}{=} L_{\mathfrak{w},\mathfrak{w}^c}$. For fixed $\mathfrak{v}$ define $[\mathfrak{v}]:=\{\mathfrak{u}\in\mathfrak{V}_k|\mathfrak{u}\sim\mathfrak{v}\}$ the equivalence class of $\mathfrak{v}$. Let $\mathfrak{v},\mathfrak{w}\in[\bar{\mathfrak{v}}]$ for some $[\bar{\mathfrak{v}}]\in\faktor{\mathfrak{V}_k}{\sim}$ and $l\in\mathbb{N}$. Then for any cycle of length $l$ from $\mathfrak{v}$ to $\mathfrak{v}$ there is a cycle from $\mathfrak{w}$ to $\mathfrak{w}$ of length $l$. Additionally, the number of distinct cycles from $\mathfrak{v}$ to $\mathfrak{v}$ equals the number of distinct cycles from $\mathfrak{w}$ to $\mathfrak{w}$. 
\end{lemma}
\begin{proof}
	The proof works constructively, based on the fact that for any neighbor $\mathfrak{u}$ of $\mathfrak{v}$ we can find a neighbor $\hat{\mathfrak{u}}$ of $\mathfrak{w}$ such that $L_{\mathfrak{u},\mathfrak{u}^c}\stackrel{\sim}{=}L_{\hat{\mathfrak{u}},\hat{\mathfrak{u}}^c}$. This allows us to iteratively construct a cycle from $\mathfrak{w}$ to $\mathfrak{w}$ based on a cycle from $\mathfrak{v}$ to $\mathfrak{v}$.\par
	For $l\in\mathbb{N}$ denote by $\phi_{\mathfrak{v}}$ a cycle from $\mathfrak{v}$ to $\mathfrak{v}$. As mentioned in the introduction, we find to $\phi_{\mathfrak{v}}(2)$ a neighbor $\mathfrak{u}$ of $\mathfrak{w}$ such that $L_{\phi_{\mathfrak{v}}(2),\phi_{\mathfrak{v}}(2)^c}\stackrel{\sim}{=}L_{\mathfrak{u},\mathfrak{u}^c}$ by replacing $w\in\mathfrak{w}$ by $u\in\mathfrak{w}^c$ where $w$ is the image of $v\in\mathfrak{v}$ and $u$ the image of $v'\in\mathfrak{v}^c$ under the isomorphism given by $L_{\mathfrak{v},\mathfrak{v}^c}\stackrel{\sim}{=}L_{\mathfrak{w},\mathfrak{w}^c}$ and $\mathfrak{v}\triangle\phi_{\mathfrak{v}}(2)=\{v,v'\}$. We call $\phi_{\mathfrak{w}}(1):=\mathfrak{w}$ and $\phi_{\mathfrak{w}}(2):=\mathfrak{u}$. Restarting the same procedure for $\phi_{\mathfrak{v}}(2)$ and $\phi_{\mathfrak{v}}(3)$ in combination with $\phi_{\mathfrak{w}}(2)$ we obtain iteratively a cycle from $\mathfrak{w}$ to $\mathfrak{w}$ and this cycle has length $l$ since otherwise there is an index $l'<l$ such that $\phi_{\mathfrak{w}}(l')=\mathfrak{w}$ and applying the previous construction to $\phi_{\mathfrak{w}}(l'-1)$ leads to $\phi_{\mathfrak{v}}(l')=\mathfrak{v}$ which is a contradiction.\par
	By the previous construction there are at least as many cycles from $\mathfrak{w}$ to $\mathfrak{w}$ as are from $\mathfrak{v}$ to $\mathfrak{v}$. But by exchanging the roles of $\mathfrak{v}$ and $\mathfrak{w}$, which is possible due to the symmetry of the equivalence relation, we obtain also the inverse sense of the inequality such that there are as many cycles from $\mathfrak{w}$ to $\mathfrak{w}$ as are from $\mathfrak{v}$ to $\mathfrak{v}$. 
\end{proof}
Based on this geometric property of $\mathfrak{L}_k$ we can analyze the stationary distribution of $\mathfrak{S}_k$ as discussed in Theorem \ref{thm:stationary_dist_level_sets_pi_k} using first return times.

==> chapters/kPG_Outlook.tex <==
Finding the vertex connectivity of a graph is a well known problem, for which fast algorithms have been developed over the years. Theorem \ref{thm:L_k_vertex_connectivity} links this topic to the topic of finding the density of the densest $k$ sub-graph of $L$. In \cite{Henzinger99361} the authors present an algorithm for finding the connectivity of a graph which is asymptotical as $\mathcal{O}(nm)$ to the number of vertices $n$ and the number of edges $m$. This implies, using Proposition \ref{prop:size_edge_set_E_k}, that there is an algorithm for finding the densest $k$ vertex induced subgraph of a $\bar{d}$-regular graph, which is asymptotical as $\mathcal{O}\left(\binom{\bar{n}}{k}^2\cdot\dfrac{\bar{d}k(\bar{n}-k)}{2(\bar{n}-1)}\right)$. Further research into this link might yield additional insights on upper bounds of the complexity of finding dense sub-graphs of regular graphs.\par
Token graphs can in general be a source of understanding for particle systems by using them as representation of the underlying state space. They have been applied, under a different name, in \cite{Fischer2022} to understand particle systems of exclusion type with various transition probabilities and the structural analysis of $\mathfrak{L}_k$ performed in hereinabove based on vertex induced subgraphs. This motivation from statistical mechanics which may even include absorbing states for particles in $L$, can be a source of motivations for further questions regarding token graphs and derived and related structures. 

==> chapters/kPG_conc.tex <==
In this first Part reviewed some basic definitions from graph and set theory as well as established in the beginning some results, in particular with a focus on sub-graphs and their role (in regular graphs). This allowed us to define the central graph theoretical object of this work, the kPG $\mathfrak{L}_k$ associated to an underlying graph $L$, as defined in Definition \ref{def:mathfrak_L_k}. We managed to formulate and proof several properties of $\mathfrak{L}_k$ on connectivtiy, the combinatorial properties, the degree sequence as well as the automorphism group, always motivated and with the application in mind, which we will discuss at length in Part \ref{part:social_net_dyna}. Hence, instead of an extensive Outlook which cannot be complete in any sens, we keep it short and let the graph theory proficient reader decide, which of the immense number of open problems they want to tackle.  

==> chapters/kPG_definition.tex <==
For any finite simple graph $L=(V,E)$ and an integer $k\in\{1,\hdots,|V|-1\}$ we consider in this work the $(L,k)$ induced sub-graph of the Johnson graph $\mathcal{J}(|V|,k)$ where $L$ is the defining structure for the edges in said graph. 
\begin{definition}[\cite{Fabila-Monroy2012}]\label{def:mathfrak_L_k}
	Consider a finite simple graph $L=(V,E)$. Define $\mathfrak{V}_k=\{\mathfrak{v}\subset v|\;|\mathfrak{v}|=k\}$ and $\mathfrak{E}_k=\{\langle\mathfrak{v},\mathfrak{w}\rangle|\mathfrak{v}\triangle\mathfrak{w}=\{v,w\};\langle v,w\rangle\in E\}$. The graph $\mathfrak{L}_k=(\mathfrak{V}_k,\mathfrak{E}_k)$  is called the $k$ Token Graph of $L$ and we denote by $\mathrm{deg}_k(\mathfrak{v})$ the degree of $\mathfrak{v}\in\mathfrak{V}_k$ in $\mathfrak{L}_k$.
\end{definition}
The graph $\mathfrak{L}_k$ as defined in Definition \ref{def:mathfrak_L_k}, based on some underlying graph $L$, has its origins in \cite{alavi1991double} and has then been considered in \cite{alavi2002survey} and then, more generally, in \cite{AUDENAERT200774} using the term \textit{symmetric $k$-th power of $L$}. A systematic analysis of these graphs has been started in \cite{Fabila-Monroy2012} under the name \textit{Token Graph}. Questions about the connectivity, cliques, the chromatic number, the spectrum and many more graph properties have been approached and answered to various extends. Most focus was put, so far for example in \cite{Fabila-Monroy2012}(\textit{connectivity, cliques, the chromatic number}), \cite{de2020independence}(\textit{Independence and matching numbers}), \cite{dalfo2021laplacian}(\textit{Laplacian spectra}) and \cite{Rivera2018Hamilton}, \cite{sym13061076}(\textit{Hamiltonicity}), on the characterizing the properties of $\mathfrak{L}_k$ via the corresponding property of the underlying graph $L$, e.g., use diameter of $L$ to bound the diameter of $\mathfrak{L}_k$ or the vertex connectivity of $L$ to make claims about the vertex connectivity of $\mathfrak{L}_k$. We change the perspective and discuss the rich structure of $\mathfrak{L}_k$ based on the vertex induced sub-graphs of $L$ and possible implications of a deeper understanding of their structure. This allows us to put its understanding in the context of particle systems of exclusion type, which opens doors to sampling based approaches which go beyond random walk based MCMC methods to access graph invariants of $L$. \par
In Figure \ref{fig:construction_L_from_C4} we show how to construct $\mathfrak{L}_k$ from an underlying graph $L$ to illustrate its structure.  
\begin{figure}[!htp]
	\centering
	\begin{tikzpicture}[scale = 0.5]
		\Vertex[x=-2,y=-2,label=$1$]{t1}
		\Vertex[x=-2,y=2,label=$2$]{t2}
		\Vertex[x=2,y=2,label=$3$]{t3}
		\Vertex[x=2,y=-2,label=$4$]{t4}
		\Edge(t1)(t2)
		\Edge(t2)(t3)
		\Edge(t3)(t4)
		\Edge(t1)(t4);
		\Vertex[x=10,y=2,size=1.2,label = {$\{1,2\}$}]{a1}
		\Vertex[x=10,y=-2,size=1.2,label = {$\{1,3\}$}]{a2}
		\Vertex[x=13,y=4,size=1.2,label = {$\{1,4\}$}]{a3}
		\Vertex[x=16,y=-2,size=1.2,label = {$\{2,3\}$}]{a4}
		\Vertex[x=16,y=2,size=1.2,label = {$\{2,4\}$}]{a5}
		\Vertex[x=13,y=-4,size=1.2,label = {$\{3,4\}$}]{a6}
		\Edge(a1)(a2)
		\Edge(a1)(a5)
		\Edge(a2)(a4)
		\Edge(a2)(a3)
		\Edge(a3)(a5)
		\Edge(a4)(a5)
		\Edge(a6)(a5)
		\Edge(a6)(a2);
		\draw[-{Latex}, ultra thick] (4,0) -- (8,0);
	\end{tikzpicture}
	\caption{Construction of $\mathfrak{L}_k$ from a $2$-regular graph on $4$ vertices for $k=2$.\label{fig:construction_L_from_C4}}
\end{figure}
Note that each vertex can be interpreted as a vertex induced sub-graph of $L$ and all edges incident to a specific vertex in $\mathfrak{L}_k$ corresponds to an edge which points outward of the induced sub-graph, as also discussed in \cite{AUDENAERT200774} and \cite{Fabila-Monroy2012}. Iterating through all vertices in $\mathfrak{L}_k$ we can reconstruct all neighborhood relationships in $L$ and, therefore, $L$ up to isomorphisms. Our focus in what follows will be on the vertex connectivity of $\mathfrak{L}_k$, its diameter in a special but still relevant case as well as the identification of cliques and the importance of the Johnson graph both as a overarching structure but also as building blocks towards maximum clique questions concerning $L$.  

==> chapters/kPG_general_prop.tex <==
We consider exclusively connected graphs $L$ throughout this work, and stay in the beginning in an unconstrained setting with respect to the degree sequence of $L$. Later on we will reduce our scope to regular graphs to obtain deeper quantitative insights. It turns out that $L$ being regular is not a strong assumption when it comes to many applications for which the graph $\mathfrak{L}_k$ reveals the deeper underlying structure.
\subsection{Geometric structure of $\mathfrak{L}_k$}
We start by the following example to motivate the role of the star graph for the understanding of the token graph. It gives an intuition on how to prove properties of $\mathfrak{L}_k$, due to the interchangeable role of all beams and the central role of the center vertex, and the fact that we can dissect any graph into many star graphs analogously to the concept of half edges.   
To illustrate our first result in a simpler context we consider first the example of the star graph, which we understand as a Corollary to Theorem \ref{thm:L_k_vertex_connectivity}, and present a short proof in this special case, which gives a first taste of the general proof structure of Theorem \ref{thm:L_k_vertex_connectivity}. The attentive reader will realize that the technique works similarly to the one used in the proof of \cite{Fabila-Monroy2012}, Lemma 3, and we will use it also in the proof of Theorem \ref{thm:L_k_vertex_connectivity}. In contrast to the proof of \cite{Fabila-Monroy2012}, Lemma 3, we stay in the realm of vertex induced sub-graphs of $L$, to make inverse claims about $L$ using $\mathfrak{L}_k$, which opens a door to computational methods using particle systems on $L$.
\begin{corollary}
	Let $L$ be the star graph on $\bar{n}+1$ vertices and $\bar{n}$ beams. Let $k\in\{1,\hdots,\bar{n}\}$. The star graph $L$ has vertex connectivity $\kappa(L)=1$ and $\mathfrak{L}_k$ satisfies
	\begin{equation}
		\kappa(\mathfrak{L}_k) = \begin{cases}
							k,& k\leq \dfrac{\bar{n}+1}{2},\vspace{5pt}\\
							\bar{n}+1-k,& k\geq \dfrac{\bar{n}+1}{2}.
						 \end{cases}
	\end{equation}		 	
\end{corollary}
\begin{proof}
	We only consider the case $k\leq \frac{\bar{n}+1}{2}$. The second case follows by $\mathfrak{L}_k\stackrel{\sim}{=}\mathfrak{L}_{\bar{n}-k}$. We denote by $\alpha$ the center of the star and by $\beta_1,\hdots,\beta_n$ the vertices at the ends of the beams. Let $\mathfrak{v}\in\mathfrak{V}_k$. We have to consider two cases, namely $\alpha\in\mathfrak{v}$ and $\alpha\not\in\mathfrak{v}$. If $\alpha\not\in\mathfrak{v}$, i.e, $\mathfrak{v}\subseteq\{\beta_1,\hdots,\beta_n\}$, then any path $(\mathfrak{v},\mathfrak{u},\mathfrak{w})$ from $\mathfrak{v}$ to $\mathfrak{w}\subseteq\{\beta_1,\hdots,\beta_n\}$ of length $2$ has to include $\alpha$ in $\mathfrak{u}$. Consequently, any $\mathfrak{v}\subseteq\{\beta_1,\hdots,\beta_n\}$ has exactly $k$ neighbors and by the same argument any $\mathfrak{v}$ containing $\alpha$ has exactly $n+1-k$ neighbors. Furthermore, for $\mathfrak{v},\mathfrak{w}\in\mathfrak{V}_k$ with $\mathfrak{v}\neq\mathfrak{w}$ and $\alpha\in\mathfrak{v}$ as well as $\alpha\in\mathfrak{w}$ we have $\langle \mathfrak{v},\mathfrak{w} \rangle\not\in\mathfrak{E}_k$. Consequently, an edge $\langle\mathfrak{v},\mathfrak{w}\rangle\in\mathfrak{E}_k$ if and only if $\alpha \in\mathfrak{v}$ and $\alpha\not\in\mathfrak{w}$ or vice versa. Therefore, as long as $\mathfrak{v}$ is connected to at least one other vertex $\mathfrak{w}$ there is a path to any other $\mathfrak{v}'\in\mathfrak{V}_k$. We conclude that the vertex connectivity is given by the minimal degree which is $\min\{k,\bar{n}+1-k\}$. This yields the claim.
\end{proof}
We find explicitly the vertex connectivity of $\mathfrak{L}_k$ for arbitrary simple connected graphs $L$.
\begin{theorem}\label{thm:L_k_vertex_connectivity}
	Let $L$ be a connected simple graph on $\bar{n}$ vertices and let $k\in\{1,\hdots,\bar{n}-1\}$. Then, $\kappa(\mathfrak{L}_k) = \min_{\mathfrak{v}\in\mathfrak{V}_k}\mathrm{deg}_k(\mathfrak{v})$ and a corresponding vertex cut is the neighborhood of $\mathfrak{v}_{\ast}\in\mathfrak{V}_k$ with $\mathrm{deg}_k(\mathfrak{v}_{\ast}) = \min_{\mathfrak{v}\in\mathfrak{V}_k}\mathrm{deg}_k(\mathfrak{v})$. 
\end{theorem}
We illustrate first the proof of Theorem \ref{thm:L_k_vertex_connectivity}. Assume we have any simple connected graph and $k=2$ particles. The proof is based on the idea of constructing marked path in $L$ and applying Menger's theorem to the ensemble of those paths. Fix to this end two configurations $\mathfrak{v}=\{v_1,v_2\}$ and $\mathfrak{w}=\{w_1,w_2\}$ which are two vertices in $\mathfrak{L}_2$. Now consider shortest paths $\phi_{v_1,w_1},\phi_{v_2,w_2}$ from $v_1$ to $w_1$ and from $v_2$ to $w_2$, respectively. We can obtain $\bar{d}-1$ distinct pairs of marked paths if either $v_1$ and $w_1$ or $v_2$ and $w_2$ are neighbors by the following construction. Assume without loss of generality that $v_1$ and $v_2$ are neighbors.
\begin{enumerate}
	\item Move the particle at $v_2$ to one of its neighbors $\tilde{v}_2$ which are not $v_1$.
	\item Move the particle at $v_1$ along $\phi_{v_1,w_1}$ to $w_1$.
	\item Move the particle at $w_1$ to any neighbor $\tilde{w}_1$ which is not $w_2$. 
	\item Move the particle at $\tilde{v}_2$ through $v_2$ along $\phi_{v_2,w_2}$ to $w_2$.
	\item Move the particle at $\tilde{w}_1$ to $w_1$. 
\end{enumerate}
Since there are $\bar{d}-1$ neighbors of $v_2$ and at least $\bar{d}-1$ neighbors of $w_1$ which allow this construction, we obtain $\bar{d}-1$ distinct pairs of marked paths. By symmetry of $v_1$ and $v_2$, we can construct exactly $2(\bar{d}-1)$ distinct pairs of marked graphs which correspond to $2(\bar{d}-1)$ paths in $\mathfrak{L}_2$. Since the minimal degree in $\mathfrak{L}_2$ is equal to $2(\bar{d}-1)$ we obtain by Menger's theorem the result given in Theorem \ref{thm:L_k_vertex_connectivity} for $k=2$ and by construction that the vertex cut is the neighborhood of the vertex in $\mathfrak{L}_2$ with minimal degree. The main challenge of the proof for arbitrary $k$ will be to rule out blockages between particles when they move along the shortest paths $\phi$ between their origin and their destination.\par
For the general case, the first point in the construction becomes "Move all particles $v_j$ but the particle at $v_i$ to one of their neighbors $\tilde{v}_j$ which are not $v_i$". The particle $v_i$ will then be moved as described before, then a second one goes to its original position, then moves and so on, iterating over all particles, the neighbors of their initial position and the neighbors of "their final position" in $\mathfrak{w}$. Note that the term "their final position" is ambiguous because the particles are indistinguishable. But this in turn allows us to fix a final position for any $v\in\mathfrak{v}$ since overlapping paths $\phi_{v_1,w_1},\phi_{v_2,w_2}$ can be rearranged into $\phi_{v_1,w_2},\phi_{v_2,w_1}$ without changing the previously discussed construction. By repeating over all sets of of neighbors by drawing without repetition and counting the number of marked paths, we obtain the result from Theorem \ref{thm:L_k_vertex_connectivity}. Furthermore, we can characterize the diameter of the $\mathfrak{L}_k$ as a function of the outer boundary of $k$ sub-graphs.
\begin{theorem}\label{thm:diameter_of_L_k}
	Let $L$ be a simple connected graph on $\bar{n}$ vertices with $\mathrm{diam}(L)=2$ and $k\in\left\{1,\hdots,\left\lfloor\frac{\bar{n}}{2}\right\rfloor\right\}$. Denote by $L_{\mathfrak{v}_{\ast}}$ the vertex induced sub-graph of $L$ on $k$ vertices $\mathfrak{v}_{\ast}\in\mathfrak{L}_k$ with the smallest outer boundary, i.e.,
	\begin{equation*}
		\mathcal{O}_b(L_{\mathfrak{v}_{\ast}}):=\left|\left(\bigcup_{v\in \mathfrak{v}_{\ast}} N_v\right)\backslash \mathfrak{v}_{\ast} \right|=\min_{\mathfrak{w}\in\mathfrak{V}_k} \left|\left(\bigcup_{w\in \mathfrak{w}} N_w\right)\backslash \mathfrak{w} \right|.
	\end{equation*}
	Define $\Delta_2^{(k)}(L):=\min\{\bar{n}-\mathcal{O}_b(L_{\mathfrak{v}_{\ast}})-k,k\}$. Then, the diameter of $\mathfrak{L}_k$ satisfies
	\begin{equation}
		\mathrm{diam}(\mathfrak{L}_k)= 2k-|k-\Delta_2(L)|=k+\Delta_2(L).
	\end{equation}
\end{theorem}
We see from the equation $\mathrm{diam}(\mathfrak{L}_k)= 2k-|k-\Delta_2(L)|$ that the crude upper of the diameter of $\mathfrak{L}_k$ by $\mathrm{diam}(L)\,k$ is only correct if $\Delta_2(L)=k$, which implies $\bar{n}-\mathcal{O}_b(L_{\mathfrak{v}_{\ast}})-k\geq k$ and, therefore, also
\begin{equation*}
	\bar{n}-2k\geq \mathcal{O}_b(L_{\mathfrak{v}_{\ast}}). 
\end{equation*} 
Even though the condition $\mathrm{diam}(L)=2$ seems restrictive at first, it does cover many interesting cases. Consider, for example two graphs $G_{1}$ and $G_{2}$ on $n$ vertices and $k$ edges. They can be interpreted as two particle configurations on the line of graph of the complete graph on $n$ vertices as depicted in Figure \ref{fig:simple_graph_to_particle_system}. 
\begin{figure}[!htb]
	\centering
	\begin{tikzpicture}[scale=0.7]
    	\Vertex[x=1,y=0, label = 1, color = white]{a}
		\Vertex[x=4,y=0, label = 2, color = white]{b}
		\Vertex[x=4,y=3, label = 3, color = white]{c}
		\Vertex[x=1,y=3, label = 4, color = white]{d}
		\Edge[color = blue,bend=-8.531](a)(c)
		\Edge[color = blue,bend=-8.531](d)(b)
		\Edge[color = blue,bend=-8.531](a)(d)
		\draw[-{Latex}, ultra thick] (5,1.5) -- (7,1.5);
		\Vertex[x=8,y=-1,size = 1,label={$\langle 1,2\rangle $}, color = white]{12}
		\Vertex[x=8,y=1.5,size = 1,label={$\langle 2,3\rangle $}, color = white]{23}
		\Vertex[x=8,y=4,size = 1,label={$\langle 3,4\rangle $}, color = white]{34}
		\Vertex[x=10,y=-1,size = 1,label={$\langle 2,4\rangle $}, color = white]{24}
		\Vertex[x=10,y=1.5,size = 1,label={$\langle 4,1\rangle $}, color = white]{41}
		\Vertex[x=10,y=4,size = 1,label={$\langle 1,3\rangle $}, color = white]{13}
		\Edge[bend=-8.531](23)(12)
		\Edge[bend=-8.531](23)(34)
		\Edge[bend=-8.531](34)(41)
		\Edge[bend=-8.531](41)(24)
		\Edge[bend=-8.531](12)(24)
		\Edge[bend=-8.531](23)(13)
		\Edge[bend=-8.531](34)(24)
		\Edge[bend=-8.531](12)(13)
		\Edge[bend=-8.531](34)(13)
		\Edge[bend=-8.531](12)(41)
		\Edge[bend=-8.531](23)(24)
		\Edge[bend=-8.531](41)(13)
		\Vertex[x=10.1,y=-0.6,color = blue,size = 0.35]{z}
		\Vertex[x=9.9,y=1.9,color = blue,size = 0.35]{z}
		\Vertex[x=10.2,y=4.4,color = blue,size = 0.35]{z}
	\end{tikzpicture}
	\caption{Transition from a simple graph on $4$ vertices and $3$ edges to a particle configuration on the line graph of the complete graph on $4$ vertices with $3$ particles.\label{fig:simple_graph_to_particle_system}}
\end{figure}
Therefore, with $\bar{n}=2^{-1}n(n-1)$ and $L$ the line graph of the complete graph on $n$ vertices, i.e., the Johnson $J(n,2)$ graph, the previous result gives a natural maximal distance between $G_{1}$ and $G_{2}$ and from the proof of the Theorem, we find even a notion of similarity for these two graphs.\par   
Since $\mathcal{O}_b(L_{\mathfrak{v}_{\ast}})$ describes the smallest outer boundary of any vertex induced sub-graph on $k$ vertices this becomes a more and more restrictive condition on the geometry of $L$ as $k$ tends to $\left\lfloor\frac{\bar{n}}{2}\right\rfloor$. This leads to the following realization.
\begin{corollary}\label{cor:star_graph_Lk_diameter}
	Let $L$ be a star graph with $\bar{n}$ beams and $k\leq \frac{\bar{n}-1}{2}$ . Then, the diameter of $\mathfrak{L}_k$ satisfies $\mathrm{diam}(\mathfrak{L}_k)= 2k$. 
\end{corollary}
The $k$ particle graph $\mathfrak{L}_k$ carries all symmetries which are also present in $L$ and $L$ is the defining object for the local and global structure of $\mathfrak{L}_k$. We can capture the implied sub-graph structures in $\mathfrak{L}_k$ combinatorically, in particular, when considering cliques in $L$. This has, in parts, been addressed in \cite{Fabila-Monroy2012}, Theorem 5.
\begin{theorem}\label{thm:cliques_in_L_Johnson_in_Lk}
	Let $L$ a simple connected graph on $\bar{n}$ vertices, $k\in\{1,\hdots,\bar{n}-1\}$ and $c\in\mathbb{N}$. Then $L$ contains a clique of size $c$ if and only if $\mathfrak{L}_k$ contains a Johnson graph $\mathcal{J}(c,k')$ for all
	\begin{equation*}
		k'\in\{\max\{1,k-(\bar{n}-c)\},\hdots,\min\{k,c-1\}\}.
	\end{equation*}
	Additionally, with $\Delta_c^L$ denoting the number of cliques of size $c$ in $L$, the number $\iota_c^{k'}$ of Johnson graphs $\mathcal{J}(c,k')$ in $\mathfrak{L}_k$ is given by
	\begin{equation}
		\iota_c^{k'} = \binom{\bar{n}-c}{k-k'}\Delta_c^L.
	\end{equation}
\end{theorem}
Using the convention that $\binom{\bar{n}}{z}=0$ for all $z\in\mathbb{Z}^-$ we obtain the following result on the clique structure of $\mathfrak{L}_k$.
\begin{theorem}\label{thm:cliques_in_Lk}
	Let $L$ a simple connected graph on $\bar{n}$ vertices, $k\in\{1,\hdots,\bar{n}-1\}$ and $c\in\mathbb{N}$. Denote by $\Delta_c^L$ the number of cliques of size $c$ in $L$, the number $\Delta_c^{\mathfrak{L}_k}$ of cliques of size $c$ in $\mathfrak{L}_k$ is given by
	\begin{equation}
		\Delta_c^{\mathfrak{L}_k} = \left(\binom{\bar{n}-c}{k-1}+\binom{\bar{n}-c}{k-(c-1)}\right)\Delta_c^L.
	\end{equation}
\end{theorem}
The identity implies directly, that there are no large cliques in $\mathfrak{L}_k$. All clique sizes in $L$ imply at most one clique size in $\mathfrak{L}_k$. In the special case of a regular graph $L$, further claims can be made.
\begin{corollary}
	If $L$ is a $\bar{d}$ regular graph, but not complete, which contains a clique of size $c$, then $\mathfrak{L}_k$ contains a clique of size $c$. 
\end{corollary}
\begin{proof}
	By Theorem \ref{thm:cliques_in_Lk} the number of cliques of size $c$ in $\mathfrak{L}_k$ is given by
	\begin{equation*}
		\Delta_c^{\mathfrak{L}_k} = \left(\binom{\bar{n}-c}{k-1}+\binom{\bar{n}-c}{k-(c-1)}\right)\Delta_c^L.
	\end{equation*}
	This term is positive if and only if $\binom{\bar{n}-c}{k-1}+\binom{\bar{n}-c}{k-(c-1)}>0$ which amounts to $k-(c-1)>0$ or $k-1<\bar{n}-c$. Assume that $k-(c-1)<0$ and $k-1>\bar{n}-c$. Then, we conclude $\frac{\bar{n}}{2}+1 < c$. Therefore, the clique has size greater then half of the vertex set but $L$ is regular and not complete such that we obtain a contradiction.
\end{proof}
We conclude with some combinatorial results for regular graphs and a link to the Johnson graph regarding the average degree of each particle. To this end, we reprove a result from \cite{Fabila-Monroy2012} on the number of edges in $\mathfrak{L}_k$, the proof giving us the necessary information need for the further discussions. 

==> chapters/kPG_general_prop_proof.tex <==
\begin{proof}[Proof Theorem \ref{thm:cliques_in_L_Johnson_in_Lk}]
	Assume that $L$ contains a clique $C$ of size $c$. Then, for $k\in\{1,n-1\}$ at least $\max\{0,k-(\bar{n}-c)\}$ tokens have to be placed inside the clique, when constructing $\mathfrak{L}_k$ and at most $\min\{c,k\}$ can be placed inside the clique. Since any Johnson graph $\mathcal{J}(c,k')$ can be seen as the token graph of the complete graph on $c$ vertices using $k'\in\{1,\hdots,c-1\}$ tokens, we see $C$ gives rise to a subgraph $\mathcal{J}(c,k')$ of $\mathfrak{L}_k$ by fixing the $k-k'$ tokens which are not contained in the clique and the $k'$ which may be placed inside under the condition that $k'\in\{\max\{1,k-(\bar{n}-c)\},\hdots,\min\{c-1,k\}\}$. \par
	On the other hand, assume that $\mathfrak{L}_k$ has for one $c\in\{1,\hdots,\bar{n}\}$ and all $k'\in\{\max\{1,k-(\bar{n}-c)\},\hdots,\min\{c-1,k\}\}$ subgraphs which are isomorphic to $\mathcal{J}(c,k')$. Then, for fixed $k'$ and one such subgraph, which we denote with some abuse of notation by $\mathcal{J}(c,k')$, we have that $\left|\bigcap_{\mathfrak{v}\in \mathcal{J}(c,k')}\mathfrak{v}\right|=k-k'$, which we may interpret as tokens which are constant over all vertices in the subgraph $\mathcal{J}(c,k')$. By this observation and the structure of the Johnson graph we find
	\begin{equation}
		\left|\left(\bigcup_{\mathfrak{w}\in \mathcal{J}(c,k')}\mathfrak{w}\right)\backslash\left(\bigcap_{\mathfrak{v}\in \mathcal{J}(c,k')}\mathfrak{v}\right)\right| = c
	\end{equation}
	and all $v\in C:=\left(\bigcup_{\mathfrak{w}\in \mathcal{J}(c,k')}\mathfrak{w}\right)\backslash\left(\bigcap_{\mathfrak{v}\in \mathcal{J}(c,k')}\mathfrak{v}\right)$ are neighbors in $L$. Hence, the subgraph spanned by $C$ is complete and $C$, therefore, a clique of $L$. The formula for the number of Johnson graphs $\mathcal{J}(c,k')$ in $\mathfrak{L}_k$, can be understood through the fact that the tokens $v\in\bigcap_{\mathfrak{v}\in \mathcal{J}(c,k')}\mathfrak{v}$ effectively give a mark in the form of a draw without replacement of size $k-k'$ to each clique whose entries are drawn from the set 
	\begin{equation}
	\mathcal{M}:=V\backslash\left(\left(\bigcup_{\mathfrak{w}\in \mathcal{J}(c,k')}\mathfrak{w}\right)\setminus\left(\bigcap_{\mathfrak{v}\in \mathcal{J}(c,k')}\mathfrak{v}\right)\right)
	\end{equation}
	and $|\mathcal{M}|=n-c$. Consequently, each clique gives rise to $\binom{n-c}{k-k'}$ marked Johnson graphs and the claim follows.
\end{proof}
We can now follow up with the proof of Theorem \ref{thm:cliques_in_Lk} which uses heavily the quantitative result on the number of Johnson graphs of fixed size. In particular, we exploit the link $\mathcal{J}(c,k')\stackrel{\sim}{=}\mathcal{J}(c,c-k')$.
\begin{proof}[Proof of Theorem \ref{thm:cliques_in_Lk}]
	Any complete graph of size $c\in\mathbb{N}$ can be identified with the Johnson graph $\mathcal{J}(c,1)$. Let $L$ be a simple connected graph on $\bar{n}$ vertices and $c\in\{1,\hdots,\bar{n}\}$. Then, both $\mathcal{J}(c,1)\stackrel{\sim}{=}K_c$ and $\mathcal{J}(c,c-1)\stackrel{\sim}{=}K_c$ form cliques in $\mathfrak{L}_k$ if $k-(\bar{n}-c)<1$ and $k>c-1$, respectively. Moreover, since for fixed $k$ and $c$, both $\mathcal{J}(c,c-1)$ and $\mathcal{J}(c,1)$ may be constructed based on a clique $C$ of size $c$ in $L$, we find $\Delta_c^{\mathfrak{L}_k}=\iota_c^{1}+\iota_c^{c-1}$. By Theorem \ref{thm:cliques_in_L_Johnson_in_Lk} and using that, we can conclude that there are 
	\begin{equation}
		\Delta_c^{\mathfrak{L}_k}=\iota_c^{1}+\iota_c^{c-1}=\binom{n-c}{k-1}\Delta_c^{L}+\binom{n-c}{k-(c-1)}\Delta_c^{L}
	\end{equation}
	cliques of size $c$ in $\mathfrak{L}_k$.
\end{proof}
The proof of Theorem \ref{thm:diameter_of_L_k} uses in the same spirit the sub-graph structure of $L$ and an inclusion-exclusion principle to prove the claim concerning the diameter of token graphs from a perspective of vertex induced subgraphs.
\begin{proof}[Proof of Theorem \ref{thm:diameter_of_L_k}]
	Since the diameter of the graph is given by a $\max$-$\min$ problem over the paths in the graph, we have to consider paths in $\mathfrak{L}_k$. In fact, this can be interpreted as moving particle systems of size $k$ on the underlying $L$. Under the assumption $\mathrm{diam}(L)=2$ we can define for any $\mathfrak{v}\in\mathfrak{V}_k$ the outer boundary of $\mathfrak{v}$ as a sub-graph of $L$ by
	\begin{equation*}
		\mathcal{O}_b(L_{\mathfrak{v}}):=\left|\left(\bigcup_{v\in \mathfrak{v}} N_v\right)\backslash \mathfrak{v}\right|.
	\end{equation*}
	These are the vertices in $L$ which are not in $\mathfrak{v}$ and for which there is a $v\in\mathfrak{v}$ such that they are neighbors. Note that possibly the set $\{w\in\mathcal{O}_b(L_{\mathfrak{v}})|\exists v\in\mathfrak{v}:d_L(v,w)=2\}$ is not empty but due to the assumption $\mathrm{diam}(L)=2$ for all $v,w\in V$ we have $d_L(v,w)\leq 2$. Consider now the set $V\backslash \left(\mathcal{A}_b(L_{\mathfrak{v}})\sqcup \mathfrak{v}\right)$ which corresponds to the set of vertices which are at distance $2$ of all $v\in\mathfrak{v}$. We write
	\begin{equation*}
		\mathcal{A}(L_{\mathfrak{v}}) = \left|V\backslash \left(\mathcal{O}_b(L_{\mathfrak{v}})\sqcup \mathfrak{v}\right)\right|=\bar{n}-\left|\mathcal{O}_b(L_{\mathfrak{v}})\right|-k.
	\end{equation*}
	Then, exactly $\mathcal{A}(L_{\mathfrak{v}})$ particles in $\mathfrak{v}$ have to be displaced at most by $2$ to attain any other configuration $\mathfrak{w}$, even at a minimal distance. Consequently, the maximal minimal distance from $\mathfrak{v}$ to any $\mathfrak{w}$ is given by
	\begin{equation*}
		\max_{\mathfrak{w}} d(\mathfrak{v},\mathfrak{w}) = 2\max\{0,\min\{k,\mathcal{A}(L_{\mathfrak{v}})\}\} + \max\{0,\min\{\bar{n}-k,k-\mathcal{A}(L_{\mathfrak{v}})\}\}.	
	\end{equation*}	  
	Note that $\mathcal{A}(L_{\mathfrak{v}})$ is maximized by $\mathfrak{v}_{\ast}$ as defined in the assumptions of the theorem and since $\max_{\mathfrak{w}} d(\mathfrak{v},\mathfrak{w})$ is monotonous in $\mathcal{A}(L_{\mathfrak{v}})$ and $\min\{k,\mathcal{A}(L_{\mathfrak{v}_{\ast}})\}=\Delta_2^{(k)}(L)$ we conclude
	\begin{equation*}
		\mathrm{diam}(\mathfrak{L}_k)=\max_{\mathfrak{v},\mathfrak{w}} d(\mathfrak{v},\mathfrak{w}) = 2\max\{0,\min\{k,\mathcal{A}(L_{\mathfrak{v}_{\ast}})\}\} + \max\{0,\min\{\bar{n}-k,k-\mathcal{A}(L_{\mathfrak{v}_{\ast}})\}\}.
	\end{equation*}
	Under the assumption $k\in\left\{1,\hdots,\left\lfloor\frac{\bar{n}}{2}\right\rfloor\right\}$ we find $\bar{n}-k\geq \left\lfloor\frac{\bar{n}}{2}\right\rfloor \geq k\geq k-\mathcal{A}(L_{\mathfrak{v}})$	and using $\Delta_2^{(k)}(L)\geq 0$, we obtain
	\begin{align*}
		\mathrm{diam}(\mathfrak{L}_k) &= 2\min\{k,\Delta_2^{(k)}(L)\} + \max\{0,k-\mathcal{A}(L_{\mathfrak{v}_{\ast}})\}\\
		&= \min\{2k,2\Delta_2^{(k)}(L)\} + k- \Delta_2^{(k)}(L)\\
		&= k + \Delta_2^{(k)}(L) -|k-\Delta_2^{(k)}(L)| + k -\Delta_2^{(k)}(L) = 2k-|k-\Delta_2^{(k)}(L)| 
	\end{align*}
	and finally, since $\Delta_2^{(k)}(L)\leq k$ we conclude $\mathrm{diam}(\mathfrak{L}_k)= k + \Delta_2^{(k)}(L)$.
\end{proof}
Finally, in Theorem \ref{thm:L_k_vertex_connectivity}, we exploit the concept of marked sub-structures of $L$, which we have already developed in the proof of Theorem \ref{thm:cliques_in_L_Johnson_in_Lk}. In said proof, we marked cliques in $L$, to count the number of subgraph in $\mathfrak{L}_k$ which are isomorphic to Johnson graphs. Now, for the proof of Theorem \ref{thm:L_k_vertex_connectivity} we extend this approach to paths, to obtain vertex disjoint paths in $\mathfrak{L}_k$ based on sets of shortest paths in $L$.
\begin{proof}[Proof of Theorem \ref{thm:L_k_vertex_connectivity}]
	Using the same construction as described before but with any number $k$ of particles, consider the initial configuration $\mathfrak{v}=\{v_1,\hdots,v_k\}$ and the finial configuration $\mathfrak{w}=\{w_1,\hdots,w_k\}$ and assume that $l$ particles $\{v_{i_1},\hdots,v_{i_l}\}$ have already been moved to neighbors $\{w_{i_1}^{(\mathfrak{n})},\hdots,w_{i_l}^{(\mathfrak{n})}\}$ of corresponding destinations $\{w_{i_1},\hdots,w_{i_l}\}$. Moreover, assume that $\{v_{i_{l+1}},\hdots,v_{i_{k-l-1}}\}$ have been moved to respective neighbors $\{v_{i_{l+1}}^{(\mathfrak{n})},\hdots,v_{i_{k-l-1}}^{(\mathfrak{n})}\}$. Finally, we want to move $v_{i_k}$ to $w_{i_k}$ along the shortest path $\phi_{v_{i_k},w_{i_k}}$. If no occupied vertices lie in $\phi_{v_{i_k},w_{i_k}}$, then nothing else has to be said. If there is an index $s$ such that $\phi_{v_{i_k},w_{i_k}}(s)$ is occupied, move $v_{i_k}$ to $\phi_{v_{i_k},w_{i_k}}(s-1)$, then move the particle in $\phi_{v_{i_k},w_{i_k}}(s)$ to $\phi_{v_{i_k},w_{i_k}}(s+1)$, then the particle which originates from $v_{i_k}$ to $\phi_{v_{i_k},w_{i_k}}(s)$ and, finally, the particle which is now in $\phi_{v_{i_k},w_{i_k}}(s+1)$ continues along $\phi_{v_{i_k},w_{i_k}}$. Since all other particles are in the neighborhood of initial or final positions, varying their positions in the respective neighborhoods leads to unique marked encounters along shortest paths. Consequently, the number of marks a single particle $v$, which moves to $w$, gives is $\min\{\mathrm{deg}(v)-\mathrm{deg}^{L_{\mathfrak{v}}}(v), \mathrm{deg}(w)-\mathrm{deg}^{L_{\mathfrak{w}}}(w)\}$. Iterating through all possible configurations of particles in neighborhoods of initial and final positions, we sum over all $v\in\mathfrak{v}$ and $w\in\mathfrak{w}$ and conclude that there are in total $\min\{\mathrm{deg}_k(\mathfrak{v}),\mathrm{deg}_k(\mathfrak{w})\}$ distinct ways to mark paths of particles in $\mathfrak{v}$ to sites in $\mathfrak{w}$. Consequently, we obtain that the number of sets of size $k$ of distinct marked paths and, therefore, the number of distinct paths in $\mathfrak{L}_k$ between $\mathfrak{v}$ and $\mathfrak{w}$ is given by $\min\{\mathrm{deg}_k(\mathfrak{v}),\mathrm{deg}_k(\mathfrak{w})\}$.\par
	Therefore, the minimal number of distinct paths between any two vertices $\mathfrak{v},\mathfrak{w}$ in $\mathfrak{L}_k$ is 
	\begin{equation}
		\min_{\mathfrak{v},\mathfrak{w}}\min\{\mathrm{deg}_k(\mathfrak{v}),\mathrm{deg}_k(\mathfrak{w})\}=\min_{\mathfrak{v}}\mathrm{deg}_k(\mathfrak{v}).
	\end{equation}
	By Menger's theorem, this yields $\kappa(\mathfrak{L}_k)=\min_{\mathfrak{v}}\mathrm{deg}_k(\mathfrak{v})$.
\end{proof}

==> chapters/kPG_intro.tex <==
Particle systems yield in the context of complex systems some accessible toy models, which allow for a reduction of the network complexity and disorder induced by the particle configuration due to an imposed crude structure. See for example \cite{10.1214/aoap/1177005359} and the discussion of the exclusion process therein, in particular the case of regular graphs, which are in spite of the richness of this class of graphs, covered by the same result. This breaks down as soon as the structure of these toy models is altered ever so slightly. This work is dedicated to the topology of graphs representing, in particular, the state space of exclusion processes with $k$ indistinguishable particles on a simple finite connected graph $L=(V,E)$. We discuss in various examples their link to random graphs and complex systems, in particular, of the social network type with dynamic relationships between individuals. These state spaces can be identified with another graph $\mathfrak{L}_k$ which represents the possible configurations of particles on the underlying simple graph. We will call $\mathfrak{L}_k$ the $k$ particle graph (kPG) to honour the particle system motivation. The vertex set of $\mathfrak{L}_k$ will be given by the $k$ subsets of $V$ neighborhood relationship in $\mathfrak{L}_k$ will be defined by the symmetric difference of two configurations which corresponds to the natural transition behavior of exclusion processes. This links $\mathfrak{L}_k$ naturally to the Johnson graph $\mathcal{J}(|V|,k)$, as defined for example in \cite{holton_sheehan_1993}, and $\mathcal{J}(|V|,k)\stackrel{=}{\sim}\mathfrak{L}_k$ if $L=L_c$ is the complete graph on $V$. Consider diagram Figure \ref{fig:diagram_L_Lk_Jnk_intro} and the links represented therein. 
\begin{figure}[!htb]
	\centering
	\begin{tikzpicture}[scale = 0.5]
		\Vertex[x=-3,y=3,label={$L$},size = 1.5]{t1}
		\Vertex[x=3,y=3,label={$L_c$},size = 1.5]{t2}
		\Vertex[x=-3,y=-3,label={$\mathfrak{L}_k$},size = 1.5]{t3}
		\Vertex[x=3,y=-3,label={$\mathcal{J}(\bar{n},k)$},size = 1.5]{t4}
		\Edge[Direct, label={$\hookrightarrow$}](t1)(t2)
		\Edge[Direct, label={$\Psi_k$}](t1)(t3)
		\Edge[Direct, label={$\Psi_k$}](t2)(t4)
		\Edge[Direct, label={$\hookrightarrow$}](t3)(t4);
	\end{tikzpicture}
	\caption{Relationships of graphs which will be discussed in what follows. The graph $L_c$ is the complete graph on the same vertex set as $L$. The map $\Psi_k$ lifts the underlying graph $L$ to the kPG using subsets of $V$ and respecting their symmetric difference.\label{fig:diagram_L_Lk_Jnk_intro}}
\end{figure}
It shows dependencies and implications of the properties of one graph and possible deductions and arguments we can formulate, by moving flexibly through the diagram. We start with the formal definition of the kPG, some related graphs, its general properties before moving on to geometric properties and quantitative results under the assumption that $L$ is regular. This assumption turns out to be weaker than it seems since it applies to important contexts in complex systems, for example the underlying state space topology of models dealing with dynamic relationships in any kind of network.


==> chapters/kPG_marked_particles.tex <==
So far, we have analyzed the structure of $\mathfrak{L}_k$ if we consider simply subsets of $V$ of size $k$. This can be seen as indistinguishable particles and we record the configurations of the particles as unordered sets in the graph $\mathfrak{L}_k$. The problem becomes more involved as soon as we make the particles distinguishable. We can, then, differentiate the particles by names or give them numbers from $1$ to $k$. This leads to a natural vertex set, which is no longer $\mathfrak{V}_k$ but $V^k$. The discussion in \cite{WILSON197486} is the basis for what follows. For $\bar{v}\in V^k$ with $\bar{v}=(\bar{v}_1,\hdots,\bar{v}_k)$ we can interpret the entry $\bar{v}_i$ as the position of particle $i$ in $L$. Note that now configurations which are permutations of one another are distinguishable. A relevant example, which shows a possible application of marked particles on some finite graph, is the $15$-puzzle. This puzzle consist of a quadratic box which can fit $16$ quadratic tiles of adequate size and $15$ small enumerated quadratic tiles which correspond to this size carrying numbers $1$ to $15$. The game then consists in ordering the tiles row by row only by sliding one tile at the time using the remaining free slot, the first row containing the numbers $1$ to $4$, the second one the numbers $5$ to $8$ and so on. One can wonder about the existence of a solution to this task depending on the initial configuration of the tiles. Indeed, this example was already of interest for the authors of \cite{Greenwell1974} and it arises now naturally as a state space in the context of interacting particles.\par
We consider a simple connected graph $L=(V,E)$ as well as $k$ occupied sites $\{v_1,\hdots,v_k\}\subset V$. For $t\geq 0$ one of the occupied sides is chosen and the occupant moves to an adjacent side uniformly chosen among the free sides. If no free sides are available the configuration remains the same.  \par
Consequently, we can associate the dynamics with exclusion process $\eta=(\eta_t)_{t\in\mathbb{N}}$ on $L$. We reformulate the exclusion process on $L$ as a Markov chain on the a sub-graph of the Hamming graph.\par
Consider the following sub-graph of the Hamming graph $\mathcal{H}(\bar{n},k)=(V_{\mathcal{H}},E_{\mathcal{H}})$ and its vertex set
\begin{equation}\label{eq:exclusive_vertex_set}
	V_{\mathcal{H}} := \{\mathrm{v}=(\mathrm{v}_1,\hdots,\mathrm{v}_k)\in \mathrm{V}^k | \forall i,j\in\{1,\hdots,k\}, i\neq j: \mathrm{v}_i \neq \mathrm{v}_j\}.
\end{equation}
Due to fact that no two entries of any vector may have the same value and, therefore, any vertex in $V_{\mathcal{H}}$ represents a subset of size $k$ of $V$, we can conclude by the same reasoning as for $\mathfrak{V}_k$ that $V_{\mathcal{H}}$ is the correct choice to capture the configurations of the exclusion process. On the other hand, the edge set of $\mathcal{H}(\bar{n},k)$ is too large, since it does not take into consideration the structure of $L$, or, it corresponds to the case where $L$ is the complete graph. Thus, we have to make the following restriction to the edge set and arrive at
\begin{equation*}
	\mathfrak{E}_k^{(\mathfrak{m})} := \{\langle v,w\rangle\in E_{\mathcal{H}} | \exists ! i,\; 1\leq i\leq k: v_i \neq w_i,\; v_j = w_j\forall j\neq i,\; \langle v_i, w_i \rangle \in E \}.
\end{equation*}
We write $\mathfrak{V}_k^{(\mathfrak{m})}:=V_{\mathcal{H}}$ and denote by $\mathfrak{L}_k^{(\mathfrak{m})} := (\mathfrak{V}_k^{(\mathfrak{m})}, \mathfrak{E}_k^{(\mathfrak{m})})$ the marked kPG associated to $L$. The graph $\mathfrak{L}_k^{(\mathfrak{m})}$ can, hence, be understood as the state space of a particle system where a transition to a different configuration corresponds to the displacement of exactly one of the $k$ particles, each particle having a distinguishable mark. \par
To construct the graph representing the state space of a $k$-particle exclusion process with marked particles we remove all nodes from $\mathcal{H}(\bar{n},k)$ for which two coordinates coincide. Naturally all edges to which such a point is incident are also being removed. For $v\in \mathfrak{V}_k^{(\mathfrak{m})}$ we denote by $\mathrm{deg}_k^{(\mathfrak{m})}(v)$ its degree in $\mathfrak{L}_k^{(\mathfrak{m})}$.\par 
Some properties of $\mathfrak{L}_k^{(\mathfrak{m})}$ may be deduced from combinatorial considerations.
\begin{lemma}\label{lem:even_degree}
	The graph $\mathfrak{L}_k^{(\mathfrak{m})}$ has the following properties.
	\begin{itemize}
		\item The vertex set $\mathfrak{V}_k^{(\mathfrak{m})}$ has size $|\mathfrak{V}_k^{(\mathfrak{m})}|=\dfrac{\bar{n}!}{(\bar{n}-k)!}$
		\item For $\mathrm{v}\in \mathfrak{V}_k^{(\mathfrak{m})}$ denote by $L_{\mathrm{v}}$ the vertex induced subgraph of $\mathrm{v}$ in $L$. Then, the degree of $\mathrm{v}$ in $\mathfrak{L}_k^{(\mathfrak{m})}$ is given by $\mathrm{deg}_k^{(\mathfrak{m})}(\mathrm{v})=\sum_{i=1}^k\mathrm{deg}(v_i)-\mathrm{deg}^{L_{\mathrm{v}}}(v_i)$.
	\end{itemize}
\end{lemma}
\begin{proof}
	Since every vertex $\mathfrak{v}\in \mathfrak{V}_k^{(\mathfrak{m})}$ may be seen as a word of length $k$ constructed from an alphabet of length $\bar{n}>k$ where each letter may be used at most once, the property 
	\begin{equation*}
		|\mathfrak{V}_k^{(\mathfrak{m})}|=\dfrac{\bar{n}!}{(\bar{n}-k)!}
	\end{equation*} 
	follows from basic combinatorial considerations on drawing without replacement.\\
	To respect the geometry of $L$, two configurations can only be neighbors if the entries which differ are connected by an edge in $L$. Hence, any $v\in\mathrm{v}$ contributes $\mathrm{deg}(v)$ to the overall degree of $\mathrm{deg}_k^{(\mathfrak{m})}(\mathrm{v})$ when we do not take into account that at most one particle may occupy any vertex in $L$. Therefore, all $k$-tuples $\mathfrak{v}\in V^k$ with multiple identical entries are removed from $V^k$ to construct $\mathfrak{V}_k^{(\mathfrak{m})}$ and each vertex $\mathfrak{w}\in \mathfrak{V}_k^{(\mathfrak{m})}$ loses all such neighbors $\mathfrak{v}$. Therefore, for any $v\in\mathrm{v}$ we obtain its final contribution to $\mathrm{deg}_k^{(\mathfrak{m})}(\mathrm{v})$ given by $\mathrm{deg}(v)-\mathrm{deg}^{L_{\mathrm{v}}}(v)$. By summing over all $v\in\mathrm{v}$ we obtain $\mathrm{deg}^{L_{\mathfrak{v}}}=\sum_{i=1}^k\mathrm{deg}(v_i)-\mathrm{deg}^{L_{\mathrm{v}}}(v_i)$.
\end{proof}
Since marked particles are not the focus of this work, we only want to give a brief insight into the differences to unmarked particles. In particular, we no longer have connectedness of $\mathfrak{L}_k^{(\mathfrak{m})}$ if $L$ is connected. In fact, this has been shown in \cite{WILSON197486} where the author gives conditions on the graphs for which connectedness follows and we can use this result due to an isomorphism which we establish in Proposition \ref{prop:Hkr_connected}.
\begin{proposition}\label{prop:Hkr_connected}
	Let $k=\bar{n}-1$. Then $\mathfrak{L}_k^{(\mathfrak{m})}\stackrel{\sim}{=}\mathrm{puz}( L )$, as defined in \cite{WILSON197486}, and is therefore connected if and only if $\mathrm{puz}( L )$ is connected.
\end{proposition}
\begin{proof}
	The existence of an isomorphism follows directly by the construction of the two objects $\mathfrak{L}_k^{(\mathfrak{m})}$ and $\mathrm{puz}( L )$.
\end{proof}
We can, therefore, use the result found in \cite{WILSON197486} to make claims about the connectivity of not only $\mathfrak{L}_k^{(\mathfrak{m})}$ but also $\mathfrak{L}_{k'}^{(\mathfrak{m})}$ for all $k'<\bar{n}-1$.
\vspace{5pt}
\begin{tcolorbox}[boxsep=0pt,arc=0pt,colback=burntorange!25!white, frame empty]%%
	\begin{proposition}\label{prop:hkr_connected}
		Let $\mathrm{puz}( L )$ be connected. For $k\leq\bar{n}-1$ the graph $\mathfrak{L}_k^{(\mathfrak{m})}$ is connected. Otherwise $\mathfrak{L}_k^{(\mathfrak{m})}$ is the empty graph. 
	\end{proposition}
\end{tcolorbox}
\begin{proof}
	We start with the second case $k\geq \bar{n}$. Again the particle interpretation helps to make the point. Assume $k=\bar{n}$. Then all sides of $ L $ are occupied by particles. Hence any vertex in $\mathfrak{L}_k^{(\mathfrak{m})}$ is only a permutation of the set of all vertices in $ L $. Moreover no particle can move which implies that there are no edges between any vertices in $\mathfrak{L}_k^{(\mathfrak{m})}$. The graph $\mathfrak{L}_k^{(\mathfrak{m})}$ is therefore the empty graph. \par
	If $k>\bar{n}$ then we find by a direct combinatorial argument that any vertex in $V_k$ contains at least one entry twice. Hence by the deletion process in the construction of $\mathfrak{V}_k^{(\mathfrak{m})}$ we obtain $\mathfrak{V}_k^{(\mathfrak{m})}=\emptyset$.\par
	Let $k' < \bar{n}$ be the number of particles on $ L $. Denote by $d':= \bar{n}-1-k'$. Then for $k:= k'+ d'$ the graph $\mathfrak{L}_k^{(\mathfrak{m})}$ is connected by Lemma \ref{prop:Hkr_connected}. Let $\nu = (\nu_1,\hdots,\nu_{k'})$ and $\tilde{\nu} = (\tilde{\nu}_1,\hdots,\tilde{\nu}_{k'})$ be some configurations. Draw $d'$ unoccupied vertices 
	\begin{equation}
		\mu_1,\hdots,\mu_{d'}\in V \backslash \{\nu_1,\hdots,\nu_{k'}\}.
	\end{equation} 
	and $d'$ vertices
	\begin{equation}
		\tilde{\mu}_1,\hdots,\tilde{\mu}_{d'}\in V \backslash \{\tilde{\nu}_1,\hdots,\tilde{\nu}_{k'}\}.
	\end{equation} 
	Consider the configurations  $\nu^{d'}= (\nu_1,\hdots,\nu_{k'},\mu_1,\hdots,\mu_{d'})$ and $\tilde{\nu}^{d'} = (\tilde{\nu}_1,\hdots,\tilde{\nu}_{k'},\tilde{\mu}_1,\hdots,\tilde{\mu}_{d'})$. Then there is a path $\phi$ in $\mathfrak{L}_k^{(\mathfrak{m})}$ connecting $\nu^{d'}$ and $\tilde{\nu}^{d'}$, from which can be constructed a path in $H_{k'}^r$ by projection on the first $k'$ components. Hence $H_{k'}^r$ is connected.
\end{proof}    
Hence, for marked particles one could use $\mathfrak{L}_k^{(\mathfrak{m})}$ and its structure to represent configurations and their connections or characterize this family of graphs in itself combinatorically. We now turn to a probabilistic application of $\mathfrak{L}_k$ for which $\mathfrak{L}_k^{(\mathfrak{m})}$ is not suited since it enforces more constraints then necessary and desired. We consider the family of processes generalized exclusion processes which describe dynamical changes of configurations of unmarked particles which are mutually exclusive, i.e., a particle cannot move to an already occupied vertex.

==> chapters/kPG_regular_graph.tex <==
In what follows we focus on regular graphs and we assume, thus, for the reminder of this section, that $L$ is a $\bar{d}$-regular graph. This allows us to state an explicit quantitative result which gives an explicit correspondence of the relationship of a regular graph with a complete graph and the associated $\mathfrak{L}_k$ with $\mathcal{J}(\bar{n},k)$.\par
We state for completeness its size which follows from standard combinatoric considerations as well as the size of the edge set, which demands a more involved analysis. 
\begin{proposition}\label{prop:size_edge_set_E_k}
	Consider the graph $\mathfrak{L}_k=(\mathfrak{V}_k, \mathfrak{E}_k)$ for $k\in\{1,\hdots,\bar{n}-1\}$. Then $|\mathfrak{V}_k|=\binom{\bar{n}}{k}$ and
	\begin{equation}\label{eq:size_of_edge_set_L_k_short}
		|\mathfrak{E}_k|=\dfrac{1}{2}\left(\bar{d}k\binom{\bar{n}}{k}-\bar{n}\bar{d}\binom{\bar{n}-2}{k-2}\right)=k(\bar{n}-k)\binom{\bar{n}}{k}\dfrac{\bar{d}}{2(\bar{n}-1)}.
	\end{equation}
\end{proposition}
\begin{proof}
	The first claim follows from drawing without replacement. For the edge set, by the formula for the degree of a $\mathfrak{v}\in\mathfrak{V}_k$, we obtain
	\begin{align*}
		2|\mathfrak{E}_k| &= \sum_{\mathfrak{v}\in\mathfrak{V}_k}\mathrm{deg}_k(\mathfrak{v})= \sum_{\mathfrak{v}\in\mathfrak{V}_k}k\bar{d}-\sum_{\mathfrak{v}\in\mathfrak{V}_k}\sum_{v\in\mathfrak{v}}\mathrm{deg}^{L_{\mathfrak{v}}}(v)\\
						  &= k\bar{d}\binom{\bar{n}}{k}-\sum_{v\in V}\sum_{\mathfrak{v}\in\mathfrak{V}_k}\mathrm{deg}^{L_{\mathfrak{v}}}(v)\mathbbm{1}_{v\in\mathfrak{v}}.
	\end{align*}
	Fixing a $v\in V$ we obtain for $s_v = \sum_{\mathfrak{v}\in\mathfrak{V}_k}\mathrm{deg}^{L_{\mathfrak{v}}}(v)\mathbbm{1}_{v\in\mathfrak{v}}$ that we have to redistribute the $k-1$ remaining particles among the $\bar{d}$ neighbors and the $\bar{n}-1-\bar{d}$ non-adjacent vertices. Assuming that $l$ particles are in the neighborhood of $\mathfrak{v}$ and one in $v$, there are $\binom{\bar{d}}{l}\binom{\bar{n}-1-\bar{d}}{k-1-l}$ ways to redistribute the particles in the aforementioned way and each contributes $l$ to to the sum $s_v$. Furthermore, $l$ ranges from $0$ to $\min\{\bar{d},k-1\}$ such that
	\begin{equation*}
		s_v = \sum_{l=0}^{\min\{\bar{d},k-1\}}\binom{\bar{d}}{l}\binom{\bar{n}-1-\bar{d}}{k-1-l}l 
	\end{equation*}		 
	independently of $v$. Consequently, we obtain the identity
	\begin{equation}\label{eq:size_of_edge_set_L_k}
			|\mathfrak{E}_k|=\dfrac{1}{2}\left(\bar{d}k\binom{\bar{n}}{k}-\bar{n}\sum_{l=1}^{\min\{k-1,\bar{d}\}}\binom{\bar{d}}{l}\binom{\bar{n}-1-\bar{d}}{k-1-l}l\right).
	\end{equation}
	For the second term, we remark that $\binom{\bar{d}}{l}=0$ for $l>\bar{d}$ and $\binom{\bar{n}-1-\bar{d}}{k-1-l}=0$ for $l>k-1$. Consequently, in the sums all summands with $l>\min\{k-1,\bar{d}\}$ are zero and, therefore,
	\begin{equation*}
		\sum_{l=1}^{k-1}\binom{\bar{d}}{l}\binom{\bar{n}-1-\bar{d}}{k-1-l}l=\sum_{l=1}^{\min\{k-1,\bar{d}\}}\binom{\bar{d}}{l}\binom{\bar{n}-1-\bar{d}}{k-1-l}l=\sum_{l=1}^{\bar{d}}\binom{\bar{d}}{l}\binom{\bar{n}-1-\bar{d}}{k-1-l}l.
	\end{equation*}
	From this we can continue with a preliminary observation that
	\begin{align*}
		\sum_{l=1}^{k-1}\binom{\bar{d}}{l}\binom{\bar{n}-1-\bar{d}}{k-1-l}l  &= \bar{d}\sum_{l=1}^{k-1}\binom{\bar{d}-1}{l-1}\binom{\bar{n}-1-\bar{d}}{k-1-l}.
	\end{align*}
	We omit $\bar{d}$ in what follows and prove only equality of the remaining terms. Note first that
	\begin{align*}
		\sum_{l=1}^{k-1}\binom{\bar{d}-1}{l-1}\binom{\bar{n}-1-\bar{d}}{k-1-l} & = \sum_{l=1}^{k-1}\binom{\bar{d}-1}{l-1}\binom{\bar{n}-2-(\bar{d}-1)}{k-2-(l-1)}\\
		& = \sum_{l=0}^{k-2}\binom{\bar{d}-1}{l}\binom{\bar{n}-2-(\bar{d}-1)}{k-2-l}
	\end{align*}
	such that we can apply the Zhu–Vandermonde identity to obtain
	\begin{align*}
		\sum_{l=1}^{k-1}\binom{\bar{d}-1}{l-1}\binom{\bar{n}-1-\bar{d}}{k-1-l} =\binom{\bar{n}-2}{k-2}
	\end{align*}
	which finishes the proof.
\end{proof}
Hence, we obtain an equality for the size of the vertex sets for $k$ and $\bar{n}-k$ as well as for the size of the edge sets in the two cases. Indeed, it is not obvious that the value given in equation \ref{eq:size_of_edge_set_L_k_short} is an integer. When checking this property one arrives at the following conclusion.
\begin{corollary}\label{cor:size_edge_set_E_k_comp_size_E}
	Let $L=(V,E)$ be a $\bar{d}$-regular graph. Consider the graph $\mathfrak{L}_k$ for $k\in\{1,\hdots,\bar{n}-1\}$. Then, 
	\begin{equation}\label{eq:size_of_edge_set_L_k_comp_L}
		|\mathfrak{E}_k|=\binom{\bar{n}-2}{k-1}|E|.
	\end{equation}
\end{corollary}
\begin{proof}
	We employ equation \ref{eq:size_of_edge_set_L_k_short} to derive the claim.
	\begin{align*}
		|\mathfrak{E}_k|&=k(\bar{n}-k)\binom{\bar{n}}{k}\dfrac{\bar{d}}{2(\bar{n}-1)}=\bar{n}\dfrac{(\bar{n}-2)!}{(k-1)!(\bar{n}-2-(k-1))!}\dfrac{\bar{d}}{2}\\
		&= \binom{\bar{n}-2}{k-1}\dfrac{\bar{n}\bar{d}}{2}=\binom{\bar{n}-2}{k-1}|E|.
	\end{align*}
\end{proof}
On the other hand comparing the result presented in equation \ref{eq:size_of_edge_set_L_k_short} with the size of the edge set $E_{\mathcal{J}}$ of a $\mathcal{J}(\bar{n},k)$ Johnson graph, we obtain that 
\begin{equation*}
	\dfrac{|\mathfrak{E}_k|}{|E_{\mathcal{J}}|}=\dfrac{\bar{d}}{\bar{n}-1}
\end{equation*} 
which is independent of $k$ and only dependent on the underlying graph $L$ through the prescribed degree $\bar{d}$. Based on this remark we can also make the following core observation for the correspondence of the relationship of a regular graph with a complete graph and the associated $\mathfrak{L}_k$ with $\mathcal{J}(\bar{n},k)$.
\begin{proposition}\label{prop:average_degree_quotient_upper_bound}
	Let $L$ be a $\bar{d}$-regular graph on $\bar{n}$ vertices and $k\in\{1,\hdots,\bar{n}-1\}$. Denote by $\mathrm{avg\;deg}(\mathfrak{L}_k)$ the average degree of $\mathfrak{L}_k$, i.e., 
	\begin{equation*}
		\mathrm{avg\;deg}(\mathfrak{L}_k):=\dfrac{1}{|\mathfrak{V}_k|}\sum_{\mathfrak{v}\in\mathfrak{V}_k}\mathrm{deg}_k(\mathfrak{v}).
	\end{equation*}
	The average degree satisfies
	\begin{equation}\label{eq:expression_quotient_average_degree}
		\dfrac{\mathrm{avg\;deg}(\mathfrak{L}_k)}{k(\bar{n}-k)}=\dfrac{\bar{d}}{\bar{n}-1}\leq 1.
	\end{equation}
\end{proposition} 
\begin{proof}
	We start by recalling that the average degree of any graph is given by the quotient of the size of its edge set times two and the size of its vertex set. Therefore,
	\begin{align*}
		\dfrac{\mathrm{avg\;deg}(\mathfrak{L}_k)}{k(\bar{n}-k)} &= \dfrac{2|\mathfrak{E}_k|}{|\mathfrak{V}_k|\,k(\bar{n}-k)}=\dfrac{\bar{d}}{\bar{n}-k} - \dfrac{\bar{d}}{\binom{\bar{n}-1}{k-1}}\dfrac{\binom{\bar{n}-2}{k-2}}{\bar{n}-k}\\
		&= \dfrac{\bar{d}}{\bar{n}-k}\left(1-\dfrac{k-1}{\bar{n}-1}\right) = \dfrac{\bar{d}}{\bar{n}-1}.
	\end{align*}
	The second claim follows from $\bar{d}\leq \bar{n}-1$ and equality if and only if $L$ is a complete graph.
\end{proof}
Consequently, by averaging over the degrees in the token graph $\mathfrak{L}_k$, we find that for an underlying $\bar{d}$ regular graph $L$ its ratio w.r.t. the degree of the $\mathcal{J}(n,k)$ is identical to the ratio of $\bar{d}$ w.r.t. the complete graph. This is, in fact, central to applications which employ particle systems, as has been done analogously classically with random walks, to identify graph properties but of higher order then those identifiable by a single particle, see also \cite{AUDENAERT200774} for a similar conceptual discussion. Some applications and first pointers are demonstrated in \cite{Fischer2022}. Further research into these links is ongoing.
\section{Special cases for $\bar{d}$-regular graph}
We discuss now special cases $\bar{d}\in\{2,\bar{n}-2\}$. In these cases, explicit quantitative statements can be made about the structure of $\mathfrak{L}_k$ for any $k\in\{1,\hdots,\bar{n}-1\}$. We consider first the case $\bar{d}=2$ and analyze the structure of the token graph $\mathfrak{L}_k$. We assume that there are $k\leq \frac{\bar{n}}{2}$ particles since by symmetry $\mathfrak{L}_k\stackrel{\sim}{=}\mathfrak{L}_{\bar{n}-k}$, as seen in \cite{AUDENAERT200774}, we cover the remaining cases as well.
\begin{proposition}\label{prop:set_D2lk_case_bar_d=2}
	Let $L$ be a cycle on $\bar{n}$ vertices and $k\in\left\{1,\hdots,\left\lfloor\frac{\bar{n}}{2}\right\rfloor\right\}$. Then, set of distinct degrees in $\mathfrak{L}_k$ is given by
	\begin{equation}
		D_k = \{2l|l\in\{1,\hdots,k\}\}.
	\end{equation}
\end{proposition}
\begin{proof}
To find the degrees in $\mathfrak{L}_k$ we can write any configuration $\mathfrak{v}$ of particles as a vector which contains as entries the size of a connected component of the vertex induced sub-graph $\mathfrak{L}_{\mathfrak{v}}$ of $\mathfrak{v}$ in $L$. Assume that there are $c'_{\mathfrak{v}}$ connected components of $\mathfrak{L}_{\mathfrak{v}}$ and denote their respective sizes by $k_i$. Each connected component contains exactly $k_i-1$ edges due to the structure of the underlying cycle graph $L$. Therefore, we obtain that 
\begin{equation*}
	\mathrm{deg}_k(\mathfrak{v}) = 2k-2\sum_{i=1}^{c'_{\mathfrak{v}}} (k_i -1) = 2 c'_{\mathfrak{v}}.
\end{equation*}
Furthermore, since $k\leq \frac{\bar{n}}{2}$ we can construct for any $l \in\{1, \hdots,k\}$ a configuration $\mathfrak{v}$ satisfying $c'_{\mathfrak{v}} = l$. This implies that $D_k = \{2l|l\in\{1,\hdots,k\}\}$.
\end{proof}
We consider now $\mathfrak{V}_{D_k;d}:=\{\mathfrak{v}\in\mathfrak{V}_k|\mathrm{deg}_k(\mathfrak{v})=d\}$. Our next task consist in finding $|\mathfrak{V}_{D_k;d}|$ for any $d\in D_k$ which is equivalent to finding the number of vertex induced $k$ sub-graphs of $L$ containing exactly $\frac{d}{2}$ edges. Indeed, this problem is equivalent to finding all unique configurations of two colored balls on a necklace with a fixed number of each color.\par
Recall that any vertex induced sub-graph $L_{\mathfrak{v}}$ can be translated to a vector of length $c'_{\mathfrak{v}}$ where each entry corresponds to the length of one connected component of $L_{\mathfrak{v}}$. We can, hence, identify the problem with finding all distinct colored necklaces of length $c'_{\mathfrak{v}}$ with colorings $\{(x_i,y_i)_{i=1}^{c'_{\mathfrak{v}}}|\sum_{i=1}^{c'_{\mathfrak{v}}}(x_i,y_i)=(k,\bar{n}-k)\}$, a problem solved by P\`olya's enumeration theorem. The number of vertex induced sub-graphs defind by each distinct necklace is then given by the size of its orbit under the symmetric group $S_{c'_{\mathfrak{v}}}$. From this we can derive $|\mathfrak{V}_{D_k;2 c'_{\mathfrak{v}}}|$ which gives the first part of the puzzle.
\begin{proposition}\label{prop:size_D2lk_case_bar_d=2}
	Let $L$ be a cycle on $\bar{n}$ vertices and $k\in\left\{1,\hdots,\left\lfloor\frac{\bar{n}}{2}\right\rfloor\right\}$. Then, for $l\in\{0,\hdots,k\}$ the identity
	\begin{equation}
		|\mathfrak{V}_{D_k;2 l}|=\binom{k-1}{l-1}\binom{\bar{n}-k-1}{l-1}\dfrac{\bar{n}}{l}
	\end{equation}
	is satisfied.
\end{proposition}
\begin{proof}
	First, note that
	\begin{align*}
		\binom{k-1}{l-1}\binom{\bar{n}-k-1}{l-1}\dfrac{\bar{n}}{l} &= \binom{k-1}{l-1}\binom{\bar{n}-k-1}{l-1}\dfrac{\bar{n}-k+k}{l}\\
		&=  \binom{k-1}{l-1}\binom{\bar{n}-k-1}{l-1}\dfrac{k}{l} + \binom{k-1}{l-1}\binom{\bar{n}-k-1}{l-1}\dfrac{\bar{n}-k}{l}\\
		&=  \binom{k}{l}\binom{\bar{n}-k-1}{l-1} + \binom{k-1}{l-1}\binom{\bar{n}-k}{l}.
	\end{align*}
	This underlines the symmetry of the problem in $k$ and $\bar{n}-k$. We cna identify the problem with counting necklaces of two colors, which are fully defined by the sets $\mathfrak{v}\in\mathfrak{V}_k$. The colors are assumed to be blue and red, where blue represents an occupied site and red an unoccupied site. We want to calculate the number of distinct blue-red colored necklaces respecting rotational symmetry, i.e., two necklaces $\mathfrak{v},\mathfrak{w}\in \mathfrak{V}_k$ are considered identical if and only if $\mathfrak{v}=\mathfrak{w}$. By fixing one vertex of the cycle, without loss of generality $v_1\in V$, we can consider necklaces starting with a blue beat, continuing then counterclockwise. \\
	Assume that $v_1$ is occupied, i.e, carries a blue beat. Place $k$ blue beats on a line of length $k$ and select $l$ of them without replacement. There are $\binom{k}{l}$. Now, separate $\bar{n}-k$ in $l$ positive parts, i.e, create a vector $(n_1,\hdots,n_l)$ with $n_i\in\mathbb{N}^{\ast}$ and $\sum_{i=1}^l n_i=\bar{n}-k$, which is possible in $\binom{\bar{n}-k-1}{l-1}$ ways. Place $n_i$ red beats after the $i$-th drawn blue beat. This construction gives, consequently, all necklaces starting with a blue beat and, thus, there are $\binom{k}{l}\binom{\bar{n}-k-1}{l-1}$ such necklaces.\\
	By symmetry there are $\binom{k-1}{l-1}\binom{\bar{n}-k}{l}$ necklaces starting with a red beat. Summing both terms yields the claim.     
\end{proof}
It turns out that the case $\bar{d}=\bar{n}-2$ is much more forgiving in terms of the difficulty of deriving $|\mathfrak{V}_{D_k;d}|$ for some fixed $d\in D_k$ which in the previous case demanded the utilization of results from combinatorics. In what follows we can reduce the problem to considerations on the graph complement of a $\bar{d}$-regular graph with $\bar{d}=\bar{n}-2$. In Figure \ref{fig:graph_complement_d_bar_equal_n_bar_minus_two} one can see the translation from the graph $L$ to its complement $L^c$ in the sens that $L^c$ contains exactly the edges which are not contained in $L$ while preserving the vertex set. This renders $L^c$ a disjoint union of paths of length $1$, exhibiting $\frac{\bar{n}}{2}$ connected components.
\begin{figure}[!htb]
	\centering
	\begin{tikzpicture}[scale = 0.8]
		\Vertex[x=0,y=0]{t1}
		\Vertex[x=-2,y=1]{t2}
		\Vertex[x=-2,y=3]{t3}
		\Vertex[x=0,y=4]{t4}
		\Vertex[x=2,y=3]{t5}
		\Vertex[x=2,y=1]{t6}
		\Edge(t1)(t2)
		\Edge(t1)(t3)
		\Edge(t1)(t6)
		\Edge(t1)(t5)
		\Edge(t2)(t3)
		\Edge(t2)(t4)
		\Edge(t2)(t5)
		\Edge(t3)(t4)
		\Edge(t3)(t6)
		\Edge(t4)(t5)
		\Edge(t4)(t6)
		\Edge(t5)(t6)
		\draw[{Latex}-{Latex}, ultra thick] (3,2) -- (6,2);
		\Vertex[x=9,y=0]{p1}
		\Vertex[x=7,y=1]{p2}
		\Vertex[x=7,y=3]{p3}
		\Vertex[x=9,y=4]{p4}
		\Vertex[x=11,y=3]{p5}
		\Vertex[x=11,y=1]{p6}
		\Edge(p1)(p4)
		\Edge(p2)(p6)
		\Edge(p3)(p5)
	\end{tikzpicture}
	\caption{Translation from the $4$-regular graph $L$ on six vertices to the disjoint union of three paths of length $1$, which corresponds to the complement graph of $L$, denoted by $L^c$. \label{fig:graph_complement_d_bar_equal_n_bar_minus_two}}
\end{figure}
\begin{proposition}\label{lem:deg_set_n_m_2}
	Let $L$ be a $\bar{n}-2$ regular graph and $k\in\left\{1,\hdots,\frac{\bar{n}}{2}\right\}$. Then,
	\begin{equation}
		D_k = \left\{k(\bar{n}-2)-k(k-1) + 2l\;\bigg|\;l\in\left\{0,\hdots,\left\lfloor\frac{k}{2}\right\rfloor\right\}\right\} 
	\end{equation}		 
	and, consequently, any degree is even.
\end{proposition}
\begin{proof}
	We employ the idea based on Figure \ref{fig:graph_complement_d_bar_equal_n_bar_minus_two} that it is sufficient to consider the graph complement $L^c$.	Let $d\in D_k$. Then there exists a $\mathfrak{v}\in\mathfrak{V}_k$ such that $\mathrm{deg}_k(\mathfrak{v}) = d$. Since $\mathfrak{v}\subset V$ it also spans a vertex induced sub-graph in $L^c$. Denote by $l$ the number of paths in $L^c$ which are fully contained in $\mathfrak{v}$, i.e., both vertices of the path are elements of $\mathfrak{v}$. Then, $l\in \left\{0,\hdots,\left\lfloor\frac{k}{2}\right\rfloor\right\}$ and 
	\begin{equation}
		d = \mathrm{deg}_k(\mathfrak{v}) = k(\bar{n}-2) -  k(k-1) + 2l.
	\end{equation}
	Since $\bar{n}-2$ is even, $k(k-1)$ is even and so is $2l$ for any positive integer $l$ we obtain that all degrees are even.
\end{proof}
Based on this correspondence between $L$ and $L^c$ we can also derive the size of each $\mathfrak{V}_{D_k;d}$ for $d\in D_k$. Additionally, we can derive $l_{\mathfrak{v}}:=|\{\mathrm{deg}_k(\mathfrak{w})|\mathrm{deg}_k(\mathfrak{w})>\mathrm{deg}_k(\mathfrak{v})\}|$. Indeed, if $\mathrm{deg}_k(\mathfrak{v})=k(\bar{n}-2) -  k(k-1) + 2l$, then $l_{\mathfrak{v}}=\left\lfloor\frac{k}{2}\right\rfloor-l$.
\begin{proposition}\label{prop:size_Deg_level_set_case_bar_d=n_2}
	Let $L$ be a $\bar{n}-2$ regular graph and $k\in\left\{1,\hdots,\frac{\bar{n}}{2}\right\}$. Then, for $j_d\in\left\{0,\hdots,\left\lfloor\frac{k}{2}\right\rfloor\right\}$ the set, corresponding to the degree $	d = k(\bar{n}-2) -  k(k-1) + 2j_d\in D_k$, satisfies the identity 
	\begin{equation}
		|\mathfrak{V}_{D_k;d}|=\sum_{l=0}^k \binom{\frac{\bar{n}}{2}}{l}\binom{l}{j_d}\binom{\frac{\bar{n}}{2}-l}{k-l-j_d}.
	\end{equation}
\end{proposition}
\begin{proof}
	Fix $j_d\in\left\{0,\hdots,\left\lfloor\frac{k}{2}\right\rfloor\right\}$. We write the vertices $v\in V$ in $\frac{\bar{n}}{2}$ columns and two rows where two vertices connected by an edge in $L^c$ belong to the same column. First, place $l$ particles in the first row. We have $\binom{\frac{\bar{n}}{2}}{l}$ possibilities to do so. To obtain a configuration $\mathfrak{v}$ with $\mathrm{deg}_k(\mathfrak{v})=k(\bar{n}-2) -  k(k-1) + 2j_d$ we have to place precisely $j_d$ of the remaining $k-l$ particles in the second row among the neighbors of the already occupied vertices. We have $\binom{l}{j_d}$ to obtain this. Finally, we distribute the remaining $k-l-j_d$ particles on the remaining $\frac{\bar{n}}{2}-l$ vertices in the second row which is possible in $\binom{\frac{\bar{n}}{2}-l}{k-l-j_d}$ ways. To obtain the total, we sum over all possibilities for $l\in\{0,\hdots,k\}$ which leads to the formula
	\begin{equation*}
		|\mathfrak{V}_{D_k;d}|=\sum_{l=0}^k \binom{\frac{\bar{n}}{2}}{l}\binom{l}{j_d}\binom{\frac{\bar{n}}{2}-l}{k-l-j_d}.
	\end{equation*}
\end{proof}
Again, these results form the basis for further approaches used in the context of sampling via particle systems, as discussed in \cite{Fischer2022}.
